Temperature Structure in the Perseus Cluster Core Observed with Hitomi

The present paper investigates the temperature structure of the X-ray emitting plasma in the core of the Perseus cluster using the 1.8--20.0 keV data obtained with the Soft X-ray Spectrometer (SXS) onboard the Hitomi Observatory. A series of four observations were carried out, with a total effective exposure time of 338 ks and covering a central region $\sim7'$ in diameter. The SXS was operated with an energy resolution of $\sim$5 eV (full width at half maximum) at 5.9 keV. Not only fine structures of K-shell lines in He-like ions but also transitions from higher principal quantum numbers are clearly resolved from Si through Fe. This enables us to perform temperature diagnostics using the line ratios of Si, S, Ar, Ca, and Fe, and to provide the first direct measurement of the excitation temperature and ionization temperature in the Perseus cluster. The observed spectrum is roughly reproduced by a single temperature thermal plasma model in collisional ionization equilibrium, but detailed line ratio diagnostics reveal slight deviations from this approximation. In particular, the data exhibit an apparent trend of increasing ionization temperature with increasing atomic mass, as well as small differences between the ionization and excitation temperatures for Fe, the only element for which both temperatures can be measured. The best-fit two-temperature models suggest a combination of 3 and 5 keV gas, which is consistent with the idea that the observed small deviations from a single temperature approximation are due to the effects of projection of the known radial temperature gradient in the cluster core along the line of sight. Comparison with the Chandra/ACIS and the XMM-Newton/RGS results on the other hand suggests that additional lower-temperature components are present in the ICM but not detectable by Hitomi SXS given its 1.8--20 keV energy band.

==> tables/fit-apec-cie.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{}
\label{}
\begin{tabular}{ccccccccccccccc}

\hline
Region/Model                           & $c$/dof       & $kT_1$                 & $Y_1$                     & $kT_2$                 & $Y_2$                     & Si                     & S                      & Ar                     & Ca                     & Cr                     & Mn                     & Fe      & Ni                     & $\sigma_v$        \\
                                       &               & (keV)                  & ($10^{14}$~cm$^{-5}$)     & (keV)                  & ($10^{14}$~cm$^{-5}$)     & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & (solar) & (solar)                & km~s$^{-1}$       \\
\hline
\hline \multicolumn{1}{l}{Entire Core} &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &         &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 13178.5/12978 & 4.00$^{+0.02}_{-0.02}$ & 0.151$^{+0.001}_{-0.001}$ & -                      & -                         & 1.07$^{+0.06}_{-0.06}$ & 1.21$^{+0.03}_{-0.03}$ & 1.10$^{+0.05}_{-0.05}$ & 1.14$^{+0.04}_{-0.04}$ & 1.06$^{+0.13}_{-0.13}$ & 1.07$^{+0.19}_{-0.19}$ & $<$0.00 & 1.00$^{+0.06}_{-0.06}$ & 145$^{+4}_{-4}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 13157.3/12976 & 4.08$^{+0.03}_{-0.03}$ & 0.146$^{+0.001}_{-0.001}$ & 1.73$^{+0.15}_{-0.11}$ & 0.012$^{+0.002}_{-0.001}$ & 0.93$^{+0.06}_{-0.06}$ & 1.11$^{+0.03}_{-0.03}$ & 1.08$^{+0.05}_{-0.05}$ & 1.14$^{+0.04}_{-0.04}$ & 1.08$^{+0.13}_{-0.13}$ & 1.08$^{+0.20}_{-0.19}$ & $<$0.00 & 1.00$^{+0.06}_{-0.06}$ & 146$^{+4}_{-4}$   \\
\multicolumn{1}{l}{\,\,\,\,9T}         & 13160.5/12971 & -                      & -                         & -                      & -                         & 0.93$^{+0.06}_{-0.06}$ & 1.10$^{+0.03}_{-0.03}$ & 1.06$^{+0.04}_{-0.04}$ & 1.12$^{+0.04}_{-0.04}$ & 1.09$^{+0.13}_{-0.13}$ & 1.08$^{+0.20}_{-0.19}$ & $<$0.00 & 1.00$^{+0.06}_{-0.06}$ & 145$^{+4}_{-4}$   \\
\hline \multicolumn{1}{l}{Nebula}      &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &         &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 12003.9/12200 & 3.91$^{+0.04}_{-0.04}$ & 0.099$^{+0.001}_{-0.001}$ & -                      & -                         & 1.10$^{+0.09}_{-0.08}$ & 1.26$^{+0.05}_{-0.05}$ & 1.14$^{+0.06}_{-0.06}$ & 1.15$^{+0.06}_{-0.05}$ & 0.91$^{+0.17}_{-0.17}$ & 1.20$^{+0.26}_{-0.26}$ & $<$0.00 & 1.10$^{+0.08}_{-0.08}$ & 150$^{+5}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 11986.8/12198 & 4.01$^{+0.10}_{-0.05}$ & 0.095$^{+0.002}_{-0.006}$ & 1.73$^{+0.41}_{-0.23}$ & 0.009$^{+0.007}_{-0.003}$ & 0.95$^{+0.08}_{-0.08}$ & 1.15$^{+0.06}_{-0.06}$ & 1.12$^{+0.06}_{-0.06}$ & 1.15$^{+0.06}_{-0.05}$ & 0.93$^{+0.18}_{-0.17}$ & 1.21$^{+0.27}_{-0.26}$ & $<$0.00 & 1.11$^{+0.08}_{-0.08}$ & 150$^{+5}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,9T}         & 11988.0/12193 & -                      & -                         & -                      & -                         & 0.95$^{+0.08}_{-0.08}$ & 1.14$^{+0.05}_{-0.06}$ & 1.11$^{+0.06}_{-0.06}$ & 1.14$^{+0.05}_{-0.05}$ & 0.94$^{+0.17}_{-0.17}$ & 1.22$^{+0.26}_{-0.26}$ & $<$0.00 & 1.11$^{+0.08}_{-0.08}$ & 150$^{+5}_{-5}$   \\
\hline \multicolumn{1}{l}{Rim}         &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &         &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 10197.0/10300 & 4.16$^{+0.04}_{-0.04}$ & 0.097$^{+0.001}_{-0.001}$ & -                      & -                         & 0.99$^{+0.11}_{-0.10}$ & 1.13$^{+0.06}_{-0.06}$ & 1.02$^{+0.08}_{-0.08}$ & 1.14$^{+0.07}_{-0.07}$ & 1.36$^{+0.21}_{-0.20}$ & 0.88$^{+0.29}_{-0.28}$ & $<$0.00 & 0.81$^{+0.08}_{-0.08}$ & 138$^{+6}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 10193.7/10298 & 4.21$^{+0.04}_{-0.04}$ & 0.095$^{+0.001}_{-0.001}$ & 1.66$^{+0.40}_{-0.28}$ & 0.004$^{+0.002}_{-0.001}$ & 0.91$^{+0.10}_{-0.09}$ & 1.07$^{+0.06}_{-0.05}$ & 1.01$^{+0.08}_{-0.07}$ & 1.14$^{+0.07}_{-0.07}$ & 1.38$^{+0.21}_{-0.20}$ & 0.88$^{+0.29}_{-0.28}$ & $<$0.00 & 0.81$^{+0.08}_{-0.08}$ & 138$^{+6}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,9T}         & 10196.3/10293 & -                      & -                         & -                      & -                         & 0.91$^{+0.10}_{-0.09}$ & 1.06$^{+0.05}_{-0.05}$ & 0.99$^{+0.07}_{-0.07}$ & 1.12$^{+0.06}_{-0.06}$ & 1.39$^{+0.21}_{-0.21}$ & 0.89$^{+0.29}_{-0.28}$ & $<$0.00 & 0.82$^{+0.08}_{-0.08}$ & 137$^{+6}_{-5}$   \\
\hline \multicolumn{1}{l}{Outer}       &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &         &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 6333.2/6929   & 5.07$^{+0.16}_{-0.15}$ & 0.027$^{+0.001}_{-0.001}$ & -                      & -                         & 1.00$^{+0.46}_{-0.40}$ & 0.92$^{+0.22}_{-0.20}$ & 1.05$^{+0.33}_{-0.31}$ & 1.42$^{+0.30}_{-0.28}$ & 1.77$^{+0.81}_{-0.76}$ & $<$1.44                & $<$0.00 & 0.99$^{+0.28}_{-0.26}$ & 160$^{+18}_{-17}$ \\
\multicolumn{1}{l}{\,\,\,\,9T}         & 6333.8/6922   & -                      & -                         & -                      & -                         & 0.99$^{+0.44}_{-0.40}$ & 0.91$^{+0.21}_{-0.22}$ & 1.04$^{+0.32}_{-0.31}$ & 1.41$^{+0.29}_{-0.28}$ & 1.78$^{-1.78}_{-0.76}$ & $<$1.44                & $<$0.00 & 0.99$^{+0.28}_{-0.26}$ & 159$^{+18}_{-17}$ \\
\hline

\end{tabular}
\end{table*}



==> tables/fit-atomdb-308-309.tex <==

\begin{table}[]
\centering

\tbl{Comparsion of the best-fit parameters between AtomDB 3.0.9 and 3.0.8}{%
\begin{tabular}{lcc}
\hline
Model/Parameter                                            & AtomDB v3.0.9           & AtomDB v3.0.8       \\
\hline \multicolumn{3}{l}{Modified 1CIE model}             \\
~~~$kT_{\mathrm{cont}}$~(keV)                              & 4.03$^{+0.01}_{-0.01}$  & 4.04$^{+0.01}_{-0.01}$  \\
~~~$kT_{\mathrm{line}}$~(keV)                              & 3.80$^{+0.02}_{-0.02}$  & 4.00$^{+0.02}_{-0.02}$  \\
~~~$Y$~(10$^{12}$~cm$^{-5}$)                               & 22.68$^{+0.04}_{-0.04}$ & 22.97$^{+0.04}_{-0.05}$ \\
~~~C-statistics/dof                                        & 13079.0/12978           & 13176.8/12978           \\
\hline \multicolumn{3}{l}{2CIE model (modified CIE + CIE)} \\
~~~$kT_{\mathrm{cont}1}$~(keV)                             & 3.66$^{+0.01}_{-0.01}$  & 4.10$^{+0.01}_{-0.01}$  \\
~~~$kT_{\mathrm{line}1}$~(keV)                             & 3.06$^{+0.03}_{-0.03}$  & 4.05$^{+0.03}_{-0.08}$  \\
~~~$kT_2$~(keV)                                            & 4.52$^{+0.02}_{-0.02}$  & 1.66$^{+0.03}_{-0.17}$  \\
~~~$Y_1$~(10$^{12}$~cm$^{-5}$)                             & 12.97$^{+0.05}_{-0.05}$ & 22.39$^{+0.06}_{-1.22}$ \\
~~~$Y_2$~(10$^{12}$~cm$^ {-5}$)                            & 9.69$^{+0.04}_{-0.04}$  & 0.88$^{+1.19}_{-1.52}$  \\
~~~C-statistics/dof                                        & 13048.9/12976           & 13168.8/12976           \\
\hline
\end{tabular}
}\label{tab:fit-compare-308-309}
\end{table}


==> tables/fit-nei-nebula.tex <==

\begin{table}[]
\centering

\caption{Best fit parameters of the 1NEI model in the Rim region}
\label{tab:fit-nei-nebula}
\begin{tabular}{lcc}
\hline
Parameter                    & AtomDB v3.0.9           & SPEXACT v3.03.00        \\
\hline
$kT$~(keV)                   & 3.92$^{+0.00}_{-0.01}$  & 3.85$^{+0.02}_{-0.02}$  \\
$kT_{\mathrm{init}}$~(keV)   & 50.0 (fixed)            & 50.0 (fixed)            \\
$nt$~(10$^{12}$~cm$^{-3}$~s) & $>$3.4                  & 2.1$^{+0.4}_{-0.2}$     \\
$Y$~(10$^{12}$~cm$^{-5}$)    & 14.98$^{+0.03}_{-0.04}$ & 20.84$^{+0.11}_{-0.11}$ \\
C-statistics/dof             & 11973.0/12200           & 12420.0/12950           \\
\hline
\end{tabular}
\end{table}


==> tables/fit-results.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{Best-fit parameters of the 1T, 2T, and NEI fits.}
\label{tab:fitting-results}
\begin{tabular}{lccccccccc}
\hline
Region  & $kT_{1}$                                                                                   & Norm$_{1}$                                                                                       & $nt_1$                                                                                     & $kT_{2}$                                                                                & Norm$_{2}$                                                                                    & $kT_{\rm cont}$                                                                                     & c-stat/d.o.f                                         \\
~~Model & (keV)                                                                                      &                                                                                                  & ($10^{12}$ ~cm$^{-3}$~s)                                                                   & (keV)                                                                                   &                                                                                               & (keV)                                                                                               &                                                      \\ \hline
Center  &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 3.87$^{+0.05}_{-0.06}$    & 5.55$^{+0.10}_{-0.09}$    & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 3.95$^{+0.04}_{-0.04}$    & 10810.9/ 11131   \\
~~2T    & 3.97$^{+0.11}_{-0.09}$    & 5.31$^{+0.22}_{-0.42}$    & $\cdots$                                                                                   & 1.72$^{+0.52}_{-0.42}$ & 0.52$^{+0.46}_{-0.25}$ & 3.96$^{+0.04}_{-0.04}$    & 10802.3/ 11129   \\
~~NEI   & 3.56$^{+0.12}_{-0.11}$ & 5.80$^{+0.13}_{-0.14}$ & 1.31$^{+0.13}_{-0.12}$ & $\cdots$                                                                                & $\cdots$                                                                                      & 3.95$^{+0.04}_{-0.04}$ & 10804.9/ 11130 \\ \hline
N       &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 4.10$^{+0.07}_{-0.07}$                   & 3.53$^{+0.07}_{-0.08}$                   & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 4.00$^{+0.04}_{-0.04}$                   & 8689.9/ 8891             \\
~~2T    & 4.16$^{+0.13}_{-0.08}$                   & 3.47$^{+0.09}_{-0.22}$                   & $\cdots$                                                                                   & 1.37$^{+0.69}_{-0.44}$                & 0.20$^{+0.23}_{-0.10}$                & 4.00$^{+0.04}_{-0.04}$                   & 8685.6/ 8889             \\
~~NEI   & 3.61$^{+0.19}_{-0.11}$                & 3.78$^{+0.07}_{-0.06}$                & 1.15$^{+0.06}_{-0.10}$                & $\cdots$                                                                                & $\cdots$                                                                                      & 4.00$^{+0.04}_{-0.04}$                & 8680.8/ 8890           \\ \hline
NW      &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 4.29$^{+0.11}_{-0.08}$                & 2.88$^{+0.07}_{-0.07}$                & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 4.17$^{+0.05}_{-0.05}$                & 8510.5/ 8688           \\
~~2T    & 4.39$^{+0.12}_{-0.13}$                & 2.78$^{+0.13}_{-0.23}$                & $\cdots$                                                                                   & 1.73$^{+0.77}_{-0.84}$             & 0.26$^{+0.23}_{-0.15}$             & 4.18$^{+0.05}_{-0.05}$                & 8505.6/ 8686           \\
~~NEI   & 3.96$^{+0.18}_{-0.08}$             & 3.01$^{+0.06}_{-0.10}$             & 1.36$^{+0.12}_{-0.09}$             & $\cdots$                                                                                & $\cdots$                                                                                      & 4.17$^{+0.04}_{-0.04}$             & 8506.7/ 8687         \\ \hline
W       &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 3.93$^{+0.05}_{-0.05}$                   & 4.46$^{+0.07}_{-0.07}$                   & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 3.90$^{+0.02}_{-0.02}$                   & 9064.1/ 9078             \\
~~2T    & 3.93$^{+0.05}_{-0.04}$                   & 4.46$^{+0.07}_{-0.07}$                   & $\cdots$                                                                                   & 1.5 (fixed)                & $<0.20$                & 3.90$^{+0.02}_{-0.02}$                   & 9064.1/ 9077             \\
~~NEI   & 3.75$^{+0.06}_{-0.04}$                & 4.56$^{+0.07}_{-0.07}$                & 1.62$^{+0.14}_{-0.12}$                & $\cdots$                                                                                & $\cdots$                                                                                      & 3.90$^{+0.02}_{-0.02}$                & 9063.7/ 9077           \\ \hline
SE      &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 4.07$^{+0.15}_{-0.14}$                & 7.36$^{+0.31}_{-0.35}$                & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 3.99$^{+0.09}_{-0.08}$                & 5580.9/ 6334           \\
~~2T    & 4.07$^{+0.14}_{-0.11}$                & 7.36$^{+0.27}_{-0.30}$                & $\cdots$                                                                                   & 1.5 (fixed)             & $<0.35$             & 3.99$^{+0.07}_{-0.07}$                & 5581.0/ 6333           \\
~~NEI   & 3.51$^{+0.25}_{-0.37}$             & 7.98$^{+0.31}_{-0.31}$             & 1.07$^{+0.12}_{-0.24}$             & $\cdots$                                                                                & $\cdots$                                                                                      & 3.99$^{+0.07}_{-0.07}$             & 5575.7/ 6333         \\ \hline
Far W   &                                                                                            &                                                                                                  &                                                                                            &                                                                                         &                                                                                               &                                                                                                     &                                                      \\
~~1T    & 5.07$^{+0.16}_{-0.15}$          & 2.45$^{+0.10}_{-0.09}$          & $\cdots$                                                                                   & $\cdots$                                                                                & $\cdots$                                                                                      & 4.86$^{+0.09}_{-0.09}$          & 6392.2/ 6911       \\
~~2T    & 5.07$^{+0.16}_{-0.14}$          & 2.45$^{+0.10}_{-0.10}$          & $\cdots$                                                                                   & 1.5 (fixed)       & $<0.44$       & 4.86$^{+0.10}_{-0.09}$          & 6392.2/ 6910       \\
~~NEI   & 5.05$^{+0.17}_{-0.27}$       & 2.43$^{+0.10}_{-0.10}$       & 4.55$^{-4.55}_{-3.02}$       & $\cdots$                                                                                & $\cdots$                                                                                      & 4.86$^{+0.09}_{-0.09}$       & 6392.0/ 6910     \\ \hline
\\
\\
\hline
Region  & Si/Fe                                                                                   & S/Fe                                                                                 & Ar/Fe                                                                                   & Ca/Fe                                                                                   & Cr/Fe                                                                                   & Mn/Fe                                                                                   & Ni/Fe                                                                                   & $v$                                                                                   \\
~~Model &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         & (km s$^{-1}$)                                                                         \\ \hline
Center  &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 1.13$^{+0.13}_{-0.12}$    & 1.32$^{+0.08}_{-0.07}$    & 1.10$^{+0.09}_{-0.09}$    & 1.24$^{+0.08}_{-0.08}$    & 0.62$^{+0.26}_{-0.26}$    & 0.92$^{+0.40}_{-0.40}$    & 1.17$^{+0.13}_{-0.13}$    & 155$^{+7}_{-8}$     \\
~~2T    & 0.97$^{+0.12}_{-0.11}$    & 1.19$^{+0.09}_{-0.08}$    & 1.07$^{+0.09}_{-0.09}$    & 1.23$^{+0.08}_{-0.08}$    & 0.63$^{+0.26}_{-0.26}$    & 0.93$^{+0.41}_{-0.40}$    & 1.17$^{+0.13}_{-0.12}$    & 155$^{+8}_{-7}$     \\
~~NEI   & 0.99$^{+0.11}_{-0.11}$ & 1.16$^{+0.09}_{-0.08}$ & 1.02$^{+0.09}_{-0.08}$ & 1.24$^{+0.08}_{-0.08}$ & 0.64$^{+0.28}_{-0.27}$ & 0.99$^{+0.44}_{-0.43}$ & 1.26$^{+0.14}_{-0.14}$ & 154$^{+7}_{-7}$  \\ \hline
N       &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 1.07$^{+0.17}_{-0.15}$                   & 1.28$^{+0.11}_{-0.09}$                   & 1.10$^{+0.12}_{-0.11}$                   & 1.20$^{+0.11}_{-0.10}$                   & 1.37$^{+0.32}_{-0.31}$                   & 1.72$^{+0.45}_{-0.43}$                   & 1.00$^{+0.13}_{-0.13}$                   & 150$^{+9}_{-9}$                    \\
~~2T    & 0.94$^{+0.17}_{-0.15}$                   & 1.21$^{+0.11}_{-0.11}$                   & 1.10$^{+0.12}_{-0.11}$                   & 1.21$^{+0.10}_{-0.10}$                   & 1.38$^{+0.32}_{-0.30}$                   & 1.73$^{+0.45}_{-0.43}$                   & 1.00$^{+0.13}_{-0.13}$                   & 151$^{+9}_{-9}$                    \\
~~NEI   & 0.87$^{+0.13}_{-0.12}$                & 1.05$^{+0.07}_{-0.07}$                & 0.98$^{+0.10}_{-0.10}$                & 1.17$^{+0.10}_{-0.09}$                & 1.54$^{+0.35}_{-0.33}$                & 1.84$^{+0.49}_{-0.47}$                & 1.11$^{+0.15}_{-0.14}$                & 147$^{+8}_{-8}$                 \\ \hline
NW      &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 1.38$^{+0.23}_{-0.20}$                & 1.22$^{+0.13}_{-0.11}$                & 0.85$^{+0.13}_{-0.13}$                & 1.09$^{+0.12}_{-0.11}$                & 1.19$^{+0.34}_{-0.33}$                & 1.08$^{+0.48}_{-0.46}$                & 0.82$^{+0.14}_{-0.13}$                & 148$^{+9}_{-9}$                 \\
~~2T    & 1.15$^{+0.22}_{-0.19}$                & 1.09$^{+0.18}_{-0.12}$                & 0.83$^{+0.15}_{-0.13}$                & 1.09$^{+0.12}_{-0.11}$                & 1.22$^{+0.35}_{-0.35}$                & 1.09$^{+0.49}_{-0.47}$                & 0.83$^{+0.14}_{-0.14}$                & 148$^{+10}_{-9}$                 \\
~~NEI   & 1.20$^{+0.18}_{-0.17}$             & 1.07$^{+0.09}_{-0.11}$             & 0.78$^{+0.12}_{-0.11}$             & 1.08$^{+0.11}_{-0.11}$             & 1.25$^{+0.36}_{-0.34}$             & 1.13$^{+0.51}_{-0.49}$             & 0.87$^{+0.15}_{-0.14}$             & 148$^{+9}_{-9}$              \\ \hline
W       &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 0.80$^{+0.13}_{-0.12}$                   & 1.06$^{+0.07}_{-0.07}$                   & 1.18$^{+0.10}_{-0.10}$                   & 1.02$^{+0.08}_{-0.08}$                   & 1.22$^{+0.27}_{-0.26}$                   & 0.62$^{+0.38}_{-0.36}$                   & 0.88$^{+0.12}_{-0.11}$                   & 127$^{+8}_{-8}$                    \\
~~2T    & 0.81$^{+0.12}_{-0.13}$                   & 1.06$^{+0.06}_{-0.08}$                   & 1.18$^{+0.10}_{-0.10}$                   & 1.02$^{+0.08}_{-0.08}$                   & 1.22$^{+0.27}_{-0.26}$                   & 0.62$^{+0.38}_{-0.36}$                   & 0.88$^{+0.12}_{-0.11}$                   & 127$^{+8}_{-8}$                    \\
~~NEI   & 0.76$^{+0.12}_{-0.11}$                & 1.00$^{+0.06}_{-0.06}$                & 1.14$^{+0.10}_{-0.09}$                & 1.02$^{+0.08}_{-0.08}$                & 1.25$^{+0.28}_{-0.27}$                & 0.66$^{+0.40}_{-0.37}$                & 0.91$^{+0.12}_{-0.11}$                & 127$^{+8}_{-8}$                 \\ \hline
SE      &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 0.76$^{+0.30}_{-0.25}$                & 1.24$^{+0.22}_{-0.18}$                & 1.21$^{+0.26}_{-0.23}$                & 1.16$^{+0.22}_{-0.20}$                & 1.07$^{+0.64}_{-0.59}$                & 1.55$^{+0.92}_{-0.85}$                & 0.87$^{+0.26}_{-0.23}$                & 138$^{+17}_{-18}$                 \\
~~2T    & 0.76$^{+0.29}_{-0.25}$                & 1.23$^{+0.17}_{-0.17}$                & 1.21$^{+0.24}_{-0.22}$                & 1.16$^{+0.21}_{-0.19}$                & 1.07$^{+0.63}_{-0.59}$                & 1.55$^{+0.91}_{-0.84}$                & 0.88$^{+0.25}_{-0.23}$                & 137$^{+17}_{-17}$                 \\
~~NEI   & 0.59$^{+0.22}_{-0.19}$             & 0.98$^{+0.13}_{-0.11}$             & 1.06$^{+0.20}_{-0.19}$             & 1.13$^{+0.19}_{-0.19}$             & 1.33$^{+0.70}_{-0.65}$             & 1.82$^{+1.03}_{-0.94}$             & 0.99$^{+0.28}_{-0.26}$             & 138$^{+17}_{-16}$              \\ \hline
Far W   &                                                                                         &                                                                                      &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                         &                                                                                       \\
~~1T    & 0.94$^{+0.46}_{-0.39}$          & 0.92$^{+0.22}_{-0.20}$          & 1.05$^{+0.33}_{-0.31}$          & 1.44$^{+0.30}_{-0.28}$          & 1.82$^{+0.81}_{-0.76}$          & 0.37$^{+1.01}_{-0.37}$          & 1.00$^{+0.28}_{-0.26}$          & 159$^{+18}_{-17}$           \\
~~2T    & 0.95$^{+0.44}_{-0.40}$          & 0.92$^{+0.22}_{-0.21}$          & 1.05$^{+0.33}_{-0.31}$          & 1.44$^{+0.30}_{-0.28}$          & 1.82$^{+0.81}_{-0.76}$          & 0.37$^{+1.01}_{-0.37}$          & 1.00$^{+0.28}_{-0.26}$          & 159$^{+18}_{-17}$           \\
~~NEI   & 0.98$^{+0.45}_{-0.42}$       & 0.95$^{+0.21}_{-0.23}$       & 1.08$^{+0.33}_{-0.33}$       & 1.47$^{+0.29}_{-0.31}$       & 1.79$^{+0.84}_{-0.75}$       & 0.35$^{+1.00}_{-0.35}$       & 0.99$^{+0.29}_{-0.26}$       & 160$^{+17}_{-18}$        \\ \hline
\end{tabular}
\end{table*}



==> tables/fit_apec_cie.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{}
\label{}
\begin{tabular}{ccccccccccccccc}
\hline
Region/Model                           & $c$/dof       & $kT_1$                 & $Y_1$                     & $kT_2$                 & $Y_2$                     & Si                     & S                      & Ar                     & Ca                     & Cr                     & Mn                     & Fe                     & Ni                     & $\sigma_v$        \\
                                       &               & (keV)                  & ($10^{14}$~cm$^{-5}$)     & (keV)                  & ($10^{14}$~cm$^{-5}$)     & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & (solar)                & km~s$^{-1}$       \\
\hline
\hline \multicolumn{1}{l}{Entire Core} &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &                        &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 13179.5/12979 & 4.03$^{+0.01}_{-0.01}$ & 0.230$^{+0.000}_{-0.000}$ & -                      & -                         & 0.72$^{+0.04}_{-0.04}$ & 0.80$^{+0.02}_{-0.02}$ & 0.72$^{+0.03}_{-0.03}$ & 0.75$^{+0.03}_{-0.03}$ & 0.70$^{+0.09}_{-0.09}$ & 0.70$^{+0.13}_{-0.12}$ & 0.65$^{+0.01}_{-0.00}$ & 0.65$^{+0.04}_{-0.04}$ & 146$^{+4}_{-4}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 13172.2/12977 & 4.07$^{+0.01}_{-0.01}$ & 0.226$^{+0.000}_{-0.000}$ & 1.62$^{+0.15}_{-0.14}$ & 0.008$^{+0.001}_{-0.001}$ & 0.68$^{+0.04}_{-0.04}$ & 0.78$^{+0.02}_{-0.02}$ & 0.73$^{+0.03}_{-0.03}$ & 0.76$^{+0.03}_{-0.03}$ & 0.71$^{+0.09}_{-0.09}$ & 0.71$^{+0.13}_{-0.13}$ & 0.66$^{+0.01}_{-0.01}$ & 0.66$^{+0.04}_{-0.04}$ & 147$^{+4}_{-4}$   \\
\hline \multicolumn{1}{l}{Nebula}      &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &                        &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 12006.1/12201 & 3.97$^{+0.02}_{-0.02}$ & 0.150$^{+0.001}_{-0.001}$ & -                      & -                         & 0.75$^{+0.06}_{-0.06}$ & 0.84$^{+0.03}_{-0.03}$ & 0.76$^{+0.04}_{-0.04}$ & 0.77$^{+0.04}_{-0.04}$ & 0.61$^{+0.11}_{-0.11}$ & 0.80$^{+0.17}_{-0.17}$ & 0.66$^{+0.01}_{-0.01}$ & 0.72$^{+0.05}_{-0.05}$ & 152$^{+5}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 12001.3/12199 & 4.00$^{+0.05}_{-0.03}$ & 0.147$^{+0.001}_{-0.004}$ & 1.41$^{+0.61}_{-0.24}$ & 0.004$^{+0.004}_{-0.002}$ & 0.71$^{+0.06}_{-0.06}$ & 0.83$^{+0.03}_{-0.04}$ & 0.77$^{+0.04}_{-0.04}$ & 0.78$^{+0.04}_{-0.04}$ & 0.62$^{+0.12}_{-0.11}$ & 0.81$^{+0.17}_{-0.17}$ & 0.66$^{+0.01}_{-0.01}$ & 0.73$^{+0.05}_{-0.05}$ & 152$^{+5}_{-5}$   \\
\hline \multicolumn{1}{l}{Rim}         &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &                        &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 10202.4/10301 & 4.07$^{+0.01}_{-0.01}$ & 0.153$^{+0.000}_{-0.000}$ & -                      & -                         & 0.62$^{+0.06}_{-0.06}$ & 0.69$^{+0.03}_{-0.03}$ & 0.63$^{+0.05}_{-0.05}$ & 0.71$^{+0.04}_{-0.04}$ & 0.85$^{+0.13}_{-0.13}$ & 0.54$^{+0.18}_{-0.18}$ & 0.64$^{+0.01}_{-0.01}$ & 0.52$^{+0.05}_{-0.05}$ & 136$^{+6}_{-5}$   \\
\multicolumn{1}{l}{\,\,\,\,2T}         & 10199.7/10299 & 5.07$^{-0.50}_{+0.50}$ & 0.026$^{-0.026}_{+0.500}$ & 3.86$^{-0.50}_{+0.50}$ & 0.129$^{-0.129}_{+0.500}$ & 0.60$^{+0.06}_{-0.06}$ & 0.67$^{+0.03}_{-0.03}$ & 0.62$^{+0.05}_{-0.05}$ & 0.70$^{+0.04}_{-0.04}$ & 0.88$^{+0.13}_{-0.13}$ & 0.56$^{+0.19}_{-0.18}$ & 0.64$^{+0.01}_{-0.01}$ & 0.52$^{+0.06}_{-0.05}$ & 136$^{+6}_{-5}$   \\
\hline \multicolumn{1}{l}{Outer}       &               &                        &                           &                        &                           &                        &                        &                        &                        &                        &                        &                        &                        &                   \\
\multicolumn{1}{l}{\,\,\,\,1T}         & 6331.3/6930   & 4.97$^{+0.08}_{-0.07}$ & 0.052$^{+0.001}_{-0.001}$ & -                      & -                         & 0.52$^{+0.22}_{-0.19}$ & 0.46$^{+0.11}_{-0.10}$ & 0.53$^{+0.17}_{-0.16}$ & 0.72$^{+0.15}_{-0.14}$ & 0.92$^{+0.42}_{-0.39}$ & $<$0.74                & 0.52$^{+0.02}_{-0.02}$ & 0.52$^{+0.15}_{-0.14}$ & 157$^{+18}_{-17}$ \\
\hline
\end{tabular}
\end{table*}


==> tables/fit_entirecore.tex <==

\begin{table}[]
\tbl{Best fit parameters for the Entire core region}{%
\centering
\begin{tabular}{lcc}
\hline
Model/Parameter                                            & AtomDB v3.0.9           & SPEXACT v3.03.00        \\
\hline
\hline \multicolumn{3}{l}{1CIE model}                      \\
~~~$kT$~(keV)                                              & 3.96$^{+0.01}_{-0.01}$  & 3.95$^{+0.01}_{-0.01}$  \\
~~~$N$~(10$^{12}$~cm$^{-5}$)                               & 23.14$^{+0.05}_{-0.05}$ & 22.72$^{+0.04}_{-0.04}$ \\
~~~C-statistics/dof                                        & 13123.0/12979           & 13176.3/12979           \\
\hline \multicolumn{3}{l}{Modified 1CIE model}             \\
~~~$kT_{\mathrm{cont}}$~(keV)                              & 4.03$^{+0.01}_{-0.01}$  & 3.97$^{+0.01}_{-0.01}$  \\
~~~$kT_{\mathrm{line}}$~(keV)                              & 3.80$^{+0.02}_{-0.02}$  & 3.89$^{+0.02}_{-0.02}$  \\
~~~$N$~(10$^{12}$~cm$^{-5}$)                               & 22.68$^{+0.04}_{-0.04}$ & 22.57$^{+0.05}_{-0.05}$ \\
~~~C-statistics/dof                                        & 13079.0/12978           & 13171.1/12978           \\
\hline \multicolumn{3}{l}{2CIE model (modified CIE + CIE)} \\
~~~$kT_{\mathrm{cont}1}$~(keV)                             & 3.66$^{+0.01}_{-0.01}$  & 3.46$^{+0.01}_{-0.02}$  \\
~~~$kT_{\mathrm{line}1}$~(keV)                             & 3.06$^{+0.03}_{-0.03}$  & 3.06$^{+0.03}_{-0.08}$  \\
~~~$kT_2$~(keV)                                            & 4.52$^{+0.02}_{-0.02}$  & 5.06$^{+0.03}_{-0.17}$  \\
~~~$N_1$~(10$^{12}$~cm$^{-5}$)                             & 12.97$^{+0.05}_{-0.05}$ & 15.59$^{+0.06}_{-0.07}$ \\
~~~$N_2$~(10$^{12}$~cm$^ {-5}$)                            & 9.69$^{+0.04}_{-0.04}$  & 7.15$^{+0.05}_{-0.06}$  \\
~~~C-statistics/dof                                        & 13048.9/12976           & 13080.0/12976           \\
\hline
\end{tabular}
}\label{tab:fit-entirecore}
\end{table}


==> tables/fit_nebularimouter.tex <==

\begin{table*}[]
\tbl{Best fit parameters for Nebula, Rim and Outer}{%
\centering
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\hline
Model/Parameter                                & \multicolumn{3}{c}{AtomDB v3.0.9} & \multicolumn{3}{c}{SPEXACT v3.03.00} \\
\cline{2-4}\cline{5-7}                         & Nebula                            & Rim                     & Outer                  & Nebula                               & Rim                     & Outer                  \\
\hline
\hline \multicolumn{7}{l}{Modified 1CIE model} \\
\hspace{0.3cm}$kT_{\mathrm{cont}}$~(keV)       & 3.98$^{+0.02}_{-0.01}$            & 4.03$^{+0.01}_{-0.01}$  & 4.93$^{+0.10}_{-0.10}$ & 3.93$^{+0.02}_{-0.02}$               & 3.97$^{+0.01}_{-0.01}$  & 4.85$^{+0.09}_{-0.09}$ \\
\hspace{0.3cm}$kT_{\mathrm{line}}$~(keV)       & 3.73$^{+0.03}_{-0.03}$            & 3.94$^{+0.04}_{-0.04}$  & 4.83$^{+0.15}_{-0.16}$ & 3.78$^{+0.06}_{-0.03}$               & 4.07$^{+0.04}_{-0.04}$  & 4.97$^{+0.16}_{-0.14}$ \\
\hspace{0.3cm}$N$~(10$^{12}$~cm$^{-5}$)        & 14.66$^{+0.06}_{-0.06}$           & 15.30$^{+0.04}_{-0.04}$ & 5.22$^{+0.10}_{-0.11}$ & 14.58$^{+0.08}_{-0.08}$              & 15.22$^{+0.04}_{-0.04}$ & 5.20$^{+0.09}_{-0.09}$ \\
~~~C-statistics/dof                            & 11934.3/12200                     & 10167.9/10300           & 6323.8/6929            & 11998.9/12200                        & 10187.5/10300           & 6326.5/6929            \\
\hline \multicolumn{7}{l}{2CIE model}          \\
\hspace{0.3cm}$kT_{\mathrm{cont}1}$~(keV)      & 3.60$^{+0.55}_{-0.06}$            & 3.65$^{+0.02}_{-0.02}$  & $\cdots$               & 3.40$^{+0.06}_{-0.09}$               & 3.40$^{+0.02}_{-0.12}$  & $\cdots$               \\
\hspace{0.3cm}$kT_{\mathrm{line}1}$~(keV)      & 2.75$^{+0.12}_{-0.43}$            & 3.47$^{+0.05}_{-0.05}$  & $\cdots$               & 2.71$^{+0.21}_{-0.26}$               & 3.27$^{+0.05}_{-0.18}$  & $\cdots$               \\
\hspace{0.3cm}$kT_2$~(keV)                     & 4.32$^{+0.03}_{-0.39}$            & 4.98$^{+0.05}_{-0.05}$  & $\cdots$               & 4.45$^{+0.34}_{-0.23}$               & 4.98$^{+0.04}_{-0.67}$  & $\cdots$               \\
\hspace{0.3cm}$N_1$~(10$^{12}$~cm$^{-5}$)      & 6.76$^{+0.58}_{-3.66}$            & 11.06$^{+0.05}_{-0.05}$ & $\cdots$               & 7.31$^{+2.02}_{-2.07}$               & 9.88$^{+0.05}_{-1.60}$  & $\cdots$               \\
\hspace{0.3cm}$N_2$~(10$^{12}$~cm$^ {-5}$)     & 7.79$^{+4.72}_{-0.56}$            & 4.38$^{+0.03}_{-0.04}$  & $\cdots$               & 7.21$^{+2.01}_{-1.94}$               & 5.52$^{+1.52}_{-0.04}$  & $\cdots$               \\
~~~C-statistics/dof                            & 11911.4/12198                     & 10161.9/10298           & $\cdots$               & 11940.0/12198                        & 10171.6/10298           & $\cdots$               \\
\hline \multicolumn{7}{l}{PSF corrected model} \\
\hspace{0.3cm}$kT_{\mathrm{cont1}}$~(keV)      & 3.72$^{+0.02}_{-0.03}$            & 3.90$^{+0.17}_{-0.17}$  & 5.11$^{+0.05}_{-0.05}$ & 3.50$^{+0.02}_{-0.02}$               & 3.94$^{+0.02}_{-0.08}$  & 5.01$^{+0.06}_{-0.05}$ \\
\hspace{0.3cm}$kT_{\mathrm{line1}}$~(keV)      & 3.00$^{+0.04}_{-0.17}$            & 3.87$^{+0.05}_{-0.12}$  & 5.00$^{+0.16}_{-0.16}$ & 2.79$^{+0.04}_{-0.03}$               & 4.13$^{+0.05}_{-0.11}$  & 5.18$^{+0.17}_{-0.16}$ \\
\hspace{0.3cm}$kT_{2}$~(keV)                   & 4.53$^{+0.05}_{-0.13}$            & 5.44$^{+0.24}_{-0.26}$  & $\cdots$               & 4.99$^{+0.05}_{-0.20}$               & $<$19.58                & $\cdots$               \\
\hspace{0.3cm}$N$~(10$^{12}$~cm$^{-5}$)        & 7.62$^{+0.04}_{-1.24}$            & 10.12$^{+0.10}_{-2.24}$ & 4.51$^{+0.04}_{-0.04}$ & 8.03$^{+0.05}_{-0.69}$               & 10.80$^{+0.08}_{-0.20}$ & 4.52$^{+0.04}_{-0.04}$ \\
\hspace{0.3cm}$N$~(10$^{12}$~cm$^{-5}$)        & 3.74$^{+1.43}_{-0.03}$            & 0.79$^{+2.65}_{-0.04}$  & $\cdots$               & 3.27$^{+0.67}_{-0.04}$               & 0.04$^{+0.04}_{-0.03}$  & $\cdots$               \\
~~~C-statistics/dof                            & ~                                 & 28391.6/29425           & ~                      & ~                                    & 28425.9/29425           & ~                      \\
\hline
\end{tabular}
}\label{tab:fitothers}
\end{table*}


==> tables/fit_nebularimouter.tex.20170804 <==

\begin{table*}[]
\centering

\caption{Best fit parameters for Neubla, Rim and Outer}
\label{tab:fitothers}
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\hline
Model/Parameter                                                & \multicolumn{3}{c}{AtomDB v3.0.8} & \multicolumn{3}{c}{SPEXACT v3.03.00} \\
\cline{2-4}\cline{5-7}                                         & Nebula                            & Rim                     & Outer                  & Nebula                               & Rim                     & Outer                  \\
\hline
\multicolumn{7}{l}{Modified 1CIE model (PSF uncorrected)}      \\
\hspace{0.3cm}$kT_{\mathrm{cont}}$~(keV)                       & 3.99$^{+0.02}_{-0.02}$            & 4.03$^{+0.01}_{-0.01}$  & 4.94$^{+0.09}_{-0.09}$ & 3.93$^{+0.02}_{-0.02}$               & 3.97$^{+0.01}_{-0.01}$  & 4.85$^{+0.09}_{-0.09}$ \\
\hspace{0.3cm}$kT_{\mathrm{line}}$~(keV)                       & 3.92$^{+0.04}_{-0.04}$            & 4.16$^{+0.04}_{-0.04}$  & 5.06$^{+0.16}_{-0.15}$ & 3.78$^{+0.06}_{-0.03}$               & 4.07$^{+0.04}_{-0.04}$  & 4.97$^{+0.16}_{-0.14}$ \\
\hspace{0.3cm}$N$~(10$^{12}$~cm$^{-5}$)                        & 14.85$^{+0.11}_{-0.11}$           & 15.48$^{+0.05}_{-0.05}$ & 5.25$^{+0.10}_{-0.09}$ & 14.58$^{+0.08}_{-0.08}$              & 15.22$^{+0.04}_{-0.04}$ & 5.20$^{+0.09}_{-0.09}$ \\
~~~C-statistics/dof                                            & 12001.7/12200                     & 10197.1/10300           & 6334.4/6929            & 11998.9/12200                        & 10187.5/10300           & 6326.5/6929            \\
\hline \multicolumn{7}{l}{Modified 1CIE model (PSF corrected)} \\
\hspace{0.3cm}$kT_{\mathrm{cont}}$~(keV)                       & 4.00$^{+0.01}_{-0.01}$            & 4.01$^{+0.02}_{-0.02}$  & 5.12$^{+0.06}_{-0.06}$ & 3.93$^{+0.01}_{-0.01}$               & 3.95$^{+0.02}_{-0.02}$  & 5.01$^{+0.06}_{-0.06}$ \\
\hspace{0.3cm}$kT_{\mathrm{line}}$~(keV)                       & 3.84$^{+0.04}_{-0.04}$            & 4.23$^{+0.05}_{-0.05}$  & 5.23$^{+0.18}_{-0.17}$ & 3.65$^{+0.03}_{-0.03}$               & 4.19$^{+0.09}_{-0.05}$  & 5.20$^{+0.17}_{-0.17}$ \\
\hspace{0.3cm}$N$~(10$^{12}$~cm$^{-5}$)                        & 11.57$^{+0.04}_{-0.04}$           & 11.00$^{+0.05}_{-0.05}$ & 4.53$^{+0.04}_{-0.04}$ & 11.34$^{+0.03}_{-0.03}$              & 10.82$^{+0.04}_{-0.04}$ & 4.52$^{+0.04}_{-0.04}$ \\
~~~C-statistics/dof                                            & $\cdots$                          & 28523.6/29429           & $\cdots$               & $\cdots$                             & 28494.0/29429           & $\cdots$               \\
\hline
\end{tabular}
\end{table*}


==> tables/lineconstraints.tex <==
\begin{table}[]
\tbl{List of lines considered in the Gaussina fit.\footnotemark[$*$]}{%
\centering
\scriptsize
\begin{tabular}{llccc}
\hline
\multicolumn{1}{c}{Line name}                            &  \multicolumn{4}{c}{Constraints}                                                \\
\cline{2-5}
                            & \multicolumn{1}{c}{Tied to}                            & \multicolumn{1}{c}{Center}                                             & \multicolumn{1}{c}{Width}                                  & \multicolumn{1}{c}{Flux}                                                \\
\hline
Si \emissiontype{XIII} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\alpha_{2}$ &   Si \emissiontype{XIV} Ly$\alpha_{1}$ &$- 1.8$ eV & $\times 1.0$  & $\times 0.5$ \\
Si \emissiontype{XIV} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\beta_{2}$ &   Si \emissiontype{XIV} Ly$\beta_{1}$ &$- 0.5$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XV} w &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\alpha_{2}$ &   S \emissiontype{XVI} Ly$\alpha_{1}$ &$- 3.0$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XVI} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\beta_{2}$ &   S \emissiontype{XVI} Ly$\beta_{1}$ &$- 0.9$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XVI} Ly$\gamma_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\gamma_{2}$ &   S \emissiontype{XVI} Ly$\gamma_{1}$ &$- 0.4$ eV & $\times 1.0$  & $\times 0.5$ \\
Ar \emissiontype{XVII} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\alpha_{2}$ &   Ar \emissiontype{XVIII} Ly$\alpha_{1}$ & $- 4.8$ eV & $\times 1.0$  & $\times 0.5$ \\
Ar \emissiontype{XVIII} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\beta_{2}$ &   Ar \emissiontype{XVIII} Ly$\beta_{1}$&$- 1.4$ eV &  $\times 1.0$ & $\times 0.5$ \\
Ca \emissiontype{XIX} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XIX} He$\beta_{1}$\footnotemark[$\dagger$] &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XX} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XX} Ly$\alpha_{2}$ &   Ca \emissiontype{XX} Ly$\alpha_{1}$&$- 7.4$ eV & $\times 1.0$  & $\times 0.5$ \\
Fe \emissiontype{XXV} z &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\beta_{2}$ &   Fe \emissiontype{XXV} He$\beta_{1}$&$- 9.5$ eV & $\times 1.0$  & - \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$ & Fe \emissiontype{XXVI} Ly$\alpha_{1}$&  - & $\times 1.0$  & - \\
Fe \emissiontype{XXVI} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXVI} Ly$\beta_{2}$ & Fe \emissiontype{XXVI} Ly$\beta_{1}$& $- 6.2$ eV & $\times 1.0$  & - \\
\hline
\multicolumn{5}{c}{Constraints only for the Rim region} \\
Si \emissiontype{XIII} w &   Si \emissiontype{XIV} Ly$\alpha_{1}$ & fixed at 1865.0 eV & $\times 1.0$  & - \\
Ca \emissiontype{XIX} He$\beta_{1}$ &  Ca \emissiontype{XX} Ly$\alpha_{1}$& fixed at 4583.5 eV &  $\times 1.0$ & - \\
\hline
\multicolumn{5}{c}{Constraints only for the Outer region} \\
Si \emissiontype{XIII} w &   Si \emissiontype{XIV} Ly$\alpha_{1}$& fixed at 1865.0 eV & $\times 1.0$  & - \\
S \emissiontype{XV} w &   S \emissiontype{XVI} Ly$\alpha_{1}$&fixed at 2460.6 eV&  $\times 1.0$ & - \\
Ca \emissiontype{XIX} He$\beta_{1}$ & Ca \emissiontype{XX} Ly$\alpha_{1}$& fixed at  4583.5 eV & $\times 1.0$  & - \\
\hline
\end{tabular}
}\label{tab:linelist}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip% 
Free parameters are denoted by the hyphen (-).
\par\noindent
\hbox to6pt{\footnotemark[$\dagger$]\hss}\unskip% 
Ca \emissiontype{XIX} He$\beta_{2}$ is omitted because it flux is $<$5\% of Ca \emissiontype{XIX} He$\beta_{1}$ for the $\sim$4~keV CIE plasma and is hard to constrain.
\end{tabnote}
\end{table}


==> tables/linefit-apec.tex <==

\begin{table}[]
\centering

\caption{}
\label{}
\begin{tabular}{ccc}

\hline
Region                          & continuum $kT$         & line $kT$              \\
                                & (keV)                  & (keV)                  \\
\hline
\multicolumn{1}{l}{Entire Core} & 4.04$^{+0.01}_{-0.01}$ & 4.00$^{+0.02}_{-0.02}$ \\
\multicolumn{1}{l}{Nebula}      & 3.99$^{+0.03}_{-0.03}$ & 3.91$^{+0.04}_{-0.04}$ \\
\multicolumn{1}{l}{Rim}         & 4.02$^{+0.01}_{-0.01}$ & 4.16$^{+0.04}_{-0.04}$ \\
\multicolumn{1}{l}{Outer}       & 4.88$^{+0.09}_{-0.09}$ & 5.07$^{+0.16}_{-0.15}$ \\
\hline

\end{tabular}
\end{table}



==> tables/lineflux.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{Observed fluxes of strong emission lines}
\label{tab:line-fluxes}
\begin{tabular}{cccccccc}
\hline
Line Name              & Fiducial Energy (eV) & \multicolumn{6}{c}{Flux (10$^{-4}$~ph~cm$^{-2}$~s$^{-1}$)}         \\ \cline{3-8} 
                       &             & Center & N & NW & W & SE & Far W \\ \hline
Si \emissiontype{XIII} w     &    1865.0        &    0.67$^{+0.35}_{-0.31}$    &  0.24$^{+0.25}_{-0.21}$  &  0.32$^{+0.25}_{-0.21}$   &   0.17$^{+0.27}_{-0.17}$ &   0.00$^{+0.68}_{-0.00}$  &    0.19$^{+0.49}_{-0.19}$    \\
Si \emissiontype{XIV} Ly$\alpha$      &    2005.5        &    1.89$^{+0.25}_{-0.24}$    &  1.21$^{+0.20}_{-0.19}$  &  1.20$^{+0.20}_{-0.19}$   &   1.27$^{+0.21}_{-0.20}$ &   2.18$^{+0.86}_{-0.74}$  &    0.56$^{+0.30}_{-0.25}$    \\
Si \emissiontype{XIV} Ly$\beta$      &    2376.3        &    0.37$^{+0.09}_{-0.08}$    &  0.22$^{+0.07}_{-0.06}$  &  0.19$^{+0.06}_{-0.06}$   &   0.21$^{+0.07}_{-0.06}$ &   0.53$^{+0.31}_{-0.27}$  &    0.19$^{+0.11}_{-0.10}$    \\
S \emissiontype{XV} w     &    2460.6        &    0.39$^{+0.07}_{-0.07}$    &  0.23$^{+0.06}_{-0.05}$  &  0.15$^{+0.05}_{-0.05}$   &   0.30$^{+0.06}_{-0.06}$ &   0.40$^{+0.24}_{-0.21}$  &    0.05$^{+0.08}_{-0.05}$    \\
S \emissiontype{XVI} Ly$\alpha$      &   2621.7        &    1.39$^{+0.08}_{-0.08}$    &  0.81$^{+0.06}_{-0.06}$  &  0.56$^{+0.05}_{-0.05}$   &   0.90$^{+0.07}_{-0.07}$ &   1.65$^{+0.28}_{-0.26}$  &    0.35$^{+0.09}_{-0.08}$    \\
S \emissiontype{XVI} Ly$\beta$      &    3106.4        &    0.21$^{+0.03}_{-0.03}$    &  0.18$^{+0.03}_{-0.01}$  &  0.14$^{+0.02}_{-0.02}$   &   0.16$^{+0.03}_{-0.03}$ &   0.31$^{+0.12}_{-0.11}$  &    0.09$^{+0.04}_{-0.03}$    \\
Ar \emissiontype{XVII} w     &    3139.6        &    0.17$^{+0.03}_{-0.03}$    &  0.11$^{+0.02}_{-0.02}$  &  0.08$^{+0.02}_{-0.02}$   &   0.10$^{+0.03}_{-0.02}$ &   0.21$^{+0.10}_{-0.09}$  &    0.12$^{+0.04}_{-0.04}$    \\
Ar \emissiontype{XVIII} Ly$\alpha$      &   3321.4        &    0.31$^{+0.03}_{-0.03}$    &  0.20$^{+0.02}_{-0.03}$  &  0.11$^{+0.02}_{-0.02}$   &   0.26$^{+0.03}_{-0.03}$ &   0.46$^{+0.11}_{-0.10}$  &    0.08$^{+0.03}_{-0.03}$    \\
Ar \emissiontype{XVIII} Ly$\beta$      &   3935.2         &    0.06$^{+0.02}_{-0.02}$    &  0.01$^{+0.01}_{-0.01}$  &  0.03$^{+0.01}_{-0.01}$   &   0.04$^{+0.01}_{-0.01}$ &   0.11$^{+0.06}_{-0.05}$  &    0.03$^{+0.02}_{-0.02}$    \\
Ca \emissiontype{XIX} w     &    3903.2        &    0.23$^{+0.02}_{-0.02}$    &  0.12$^{+0.02}_{-0.02}$  &  0.10$^{+0.01}_{-0.01}$   &   0.16$^{+0.02}_{-0.02}$ &   0.16$^{+0.06}_{-0.06}$  &    0.08$^{+0.02}_{-0.02}$    \\
Ca \emissiontype{XIX} He$\beta$      &    4575.6        &    0.23$^{+0.02}_{-0.02}$    &  0.12$^{+0.02}_{-0.02}$  &  0.10$^{+0.01}_{-0.01}$   &   0.16$^{+0.02}_{-0.02}$ &   0.16$^{+0.06}_{-0.06}$  &    0.08$^{+0.02}_{-0.02}$    \\
Ca \emissiontype{XX} Ly$\alpha$      &   4105.0       &    0.13$^{+0.02}_{-0.02}$    &  0.12$^{+0.02}_{-0.02}$  &  0.06$^{+0.01}_{-0.01}$   &   0.09$^{+0.01}_{-0.01}$ &   0.27$^{+0.07}_{-0.07}$  &    0.09$^{+0.02}_{-0.02}$    \\
Fe \emissiontype{XXV} z     &    6636.6        &    0.54$^{+0.02}_{-0.02}$    &  0.37$^{+0.02}_{-0.02}$  &  0.29$^{+0.01}_{-0.01}$   &   0.38$^{+0.02}_{-0.02}$ &   0.74$^{+0.07}_{-0.06}$  &    0.30$^{+0.03}_{-0.03}$    \\
Fe \emissiontype{XXV} w     &    6700.4        &    1.22$^{+0.03}_{-0.03}$    &  0.85$^{+0.02}_{-0.02}$  &  0.70$^{+0.02}_{-0.02}$   &   0.99$^{+0.03}_{-0.02}$ &   1.68$^{+0.09}_{-0.09}$  &    0.88$^{+0.04}_{-0.04}$    \\
Fe \emissiontype{XXV} He$\beta$      &   7881.5        &    0.19$^{+0.01}_{-0.01}$    &  0.12$^{+0.01}_{-0.01}$  &  0.11$^{+0.01}_{-0.01}$   &   0.14$^{+0.01}_{-0.01}$ &   0.18$^{+0.04}_{-0.03}$  &    0.13$^{+0.02}_{-0.02}$    \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$      &   6973.1       &    0.12$^{+0.01}_{-0.01}$    &  0.09$^{+0.01}_{-0.01}$  &  0.09$^{+0.01}_{-0.01}$   &   0.10$^{+0.01}_{-0.01}$ &   0.20$^{+0.04}_{-0.03}$  &    0.11$^{+0.02}_{-0.02}$    \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$      &   6951.9       &    0.06$^{+0.01}_{-0.01}$    &  0.05$^{+0.01}_{-0.01}$  &  0.05$^{+0.01}_{-0.01}$   &   0.07$^{+0.01}_{-0.01}$ &   0.11$^{+0.03}_{-0.03}$  &    0.08$^{+0.02}_{-0.02}$    \\
Fe \emissiontype{XXVI} Ly$\beta$      &   8250.5         &    0.02$^{+0.01}_{-0.01}$    &  0.01$^{+0.01}_{-0.00}$  &  0.02$^{+0.01}_{-0.01}$   &   0.01$^{+0.01}_{-0.00}$ &   0.02$^{+0.03}_{-0.02}$  &    0.02$^{+0.01}_{-0.01}$    \\ \hline
\end{tabular}
\end{table*}




==> tables/linefluxnew.tex.20170719 <==
\begin{landscape}
\begin{table}[]
\tbl{Results of the Gaussian fits.\footnotemark[$*$]}{%
\centering
\scriptsize
\begin{tabular}{cccccccccccccccc}
\hline
Line name                              & Energy (eV) & \multicolumn{4}{c}{Center (eV)} &   & \multicolumn{4}{c}{Width (eV)} &   & \multicolumn{4}{c}{Flux (10$^{-5}$~ph~cm$^{-2}$~s$^{-1}$)} \\
\cline{3-6}\cline{8-11}\cline{13-16}   &             & Entire Core                     & Nebula                 & Rim                    & Outer                     & ~ & Entire Core                    & Nebula              & Rim                 & Outer                 & ~ & Entire Core                                                & Nebula                  & Rim                     & Outer                  \\
\hline
Si \emissiontype{XIII} w               & 1865.0      & 1864.6$^{+1.0}_{-1.1}$          & 1864.2$^{+1.5}_{-1.0}$ & (fixed)                & (fixed)                   &   & $<$1.7                         & $<$1.7              & (tied)              & (tied)                &   & 7.19$^{+3.77}_{-3.42}$                                     & 5.83$^{+3.63}_{-2.51}$  & $<$5.44                 & $<$4.58                \\
Si \emissiontype{XIV} Ly$\alpha_{1}$   & 2006.1      & 2006.4$^{+0.3}_{-0.2}$          & 2006.5$^{+0.3}_{-0.2}$ & 2006.4$^{+0.4}_{-0.3}$ & 2006.4$^{+1.4}_{-1.4}$    &   & 1.3$^{+0.3}_{-0.3}$            & $<$1.5              & 1.7$^{+0.5}_{-0.5}$ & $<$2.8                &   & 31.90$^{+2.28}_{-2.21}$                                    & 20.10$^{+1.92}_{-1.82}$ & 21.82$^{+2.64}_{-2.52}$ & 4.04$^{+2.09}_{-1.67}$ \\
Si \emissiontype{XIV} Ly$\beta_{1}$    & 2376.6      & 2376.5$^{+0.5}_{-0.5}$          & 2376.2$^{+0.5}_{-0.5}$ & 2377.8$^{+1.3}_{-1.4}$ & 2378.5$^{+1.0}_{-1.4}$    &   & 2.4$^{+0.5}_{-0.5}$            & 2.2$^{+0.5}_{-0.5}$ & 3.8$^{+1.3}_{-1.2}$ & $<$2.0                &   & 6.89$^{+0.89}_{-0.86}$                                     & 5.03$^{+0.74}_{-0.70}$  & 3.93$^{+1.04}_{-0.98}$  & 1.23$^{+0.80}_{-0.60}$ \\
S \emissiontype{XV} w                  & 2460.6      & 2460.7$^{+0.5}_{-0.3}$          & 2460.6$^{+0.6}_{-0.4}$ & 2460.7$^{+0.8}_{-0.6}$ & (fixed)                   &   & 2.1$^{+0.6}_{-0.6}$            & 2.6$^{+0.8}_{-0.7}$ & $<$2.2              & (tied)                &   & 9.21$^{+1.10}_{-1.11}$                                     & 7.26$^{+0.98}_{-0.99}$  & 3.91$^{+1.03}_{-0.94}$  & $<$1.08                \\
S \emissiontype{XVI} Ly$\alpha_{1}$    & 2622.7      & 2622.6$^{+0.1}_{-0.1}$          & 2622.7$^{+0.1}_{-0.2}$ & 2622.6$^{+0.2}_{-0.2}$ & 2621.6$^{+0.9}_{-0.9}$    &   & 1.8$^{+0.2}_{-0.2}$            & 1.9$^{+0.2}_{-0.2}$ & 1.7$^{+0.3}_{-0.3}$ & 2.0$^{+1.0}_{-1.1}$   &   & 22.32$^{+0.73}_{-0.72}$                                    & 15.81$^{+0.64}_{-0.63}$ & 12.46$^{+0.77}_{-0.76}$ & 2.70$^{+0.68}_{-0.61}$ \\
S \emissiontype{XVI} Ly$\beta_{1}$     & 3106.7      & 3106.4$^{+0.3}_{-0.3}$          & 3106.0$^{+0.4}_{-0.4}$ & 3107.0$^{+0.3}_{-0.5}$ & 3116.1$^{+0.7}_{-1.3}$    &   & 2.1$^{+0.4}_{-0.3}$            & 2.4$^{+0.5}_{-0.4}$ & 1.8$^{+0.5}_{-0.7}$ & $<$1.8                &   & 3.83$^{+0.29}_{-0.29}$                                     & 2.55$^{+0.25}_{-0.24}$  & 2.49$^{+0.34}_{-0.33}$  & 0.63$^{+0.26}_{-0.23}$ \\
S \emissiontype{XVI} Ly$\gamma_{1}$    & 3276.3      & 3276.8$^{+0.3}_{-0.8}$          & 3276.8$^{+0.4}_{-0.9}$ & 3276.3$^{+1.0}_{-0.8}$ & 3275.7$^{+1.4}_{-1.5}$    &   & $<$2.0                         & $<$2.4              & 1.8$^{+1.2}_{-1.4}$ & $<$2.4                &   & 1.20$^{+0.20}_{-0.19}$                                     & 0.79$^{+0.09}_{-0.25}$  & 0.92$^{+0.25}_{-0.24}$  & 0.32$^{+0.22}_{-0.17}$ \\
Ar \emissiontype{XVII} w               & 3139.6      & 3139.5$^{+0.3}_{-0.3}$          & 3139.5$^{+0.3}_{-0.4}$ & 3139.3$^{+1.2}_{-1.1}$ & 3142.4$^{+0.7}_{-0.9}$    &   & 1.5$^{+0.4}_{-0.4}$            & 1.1$^{+0.5}_{-0.6}$ & 3.0$^{+1.4}_{-1.1}$ & $<$1.9                &   & 3.72$^{+0.37}_{-0.36}$                                     & 2.82$^{+0.31}_{-0.30}$  & 1.88$^{+0.51}_{-0.47}$  & 1.20$^{+0.42}_{-0.34}$ \\
Ar \emissiontype{XVIII} Ly$\alpha_{1}$ & 3323.0      & 3322.9$^{+0.2}_{-0.3}$          & 3323.1$^{+0.3}_{-0.4}$ & 3322.5$^{+0.5}_{-0.4}$ & 3326.6$^{+2.2}_{-2.2}$    &   & 2.7$^{+0.4}_{-0.4}$            & 3.0$^{+0.4}_{-0.4}$ & 2.2$^{+0.6}_{-0.6}$ & 4.2$^{+2.3}_{-1.6}$   &   & 5.47$^{+0.29}_{-0.29}$                                     & 3.85$^{+0.25}_{-0.25}$  & 3.16$^{+0.32}_{-0.30}$  & 0.95$^{+0.32}_{-0.30}$ \\
Ar \emissiontype{XVIII} Ly$\beta_{1}$  & 3935.7      & 3935.0$^{+0.9}_{-1.0}$          & 3936.2$^{+0.7}_{-1.3}$ & 3931.4$^{+1.5}_{-1.7}$ & 3946.6$^{+0.7}_{-1.2}$    &   & 2.8$^{+1.0}_{-0.8}$            & 2.3$^{+1.0}_{-0.9}$ & 3.7$^{+1.7}_{-1.6}$ & $<$1.2                &   & 0.77$^{+0.15}_{-0.15}$                                     & 0.51$^{+0.12}_{-0.12}$  & 0.63$^{+0.20}_{-0.18}$  & 0.26$^{+0.15}_{-0.11}$ \\
Ca \emissiontype{XIX} w                & 3902.4      & 3902.4$^{+0.2}_{-0.2}$          & 3902.5$^{+0.2}_{-0.3}$ & 3902.1$^{+0.3}_{-0.4}$ & 3902.4$^{+1.5}_{-1.1}$    &   & 2.3$^{+0.2}_{-0.2}$            & 2.4$^{+0.3}_{-0.3}$ & 2.2$^{+0.4}_{-0.4}$ & 2.7$^{+1.5}_{-1.2}$   &   & 5.20$^{+0.27}_{-0.27}$                                     & 3.66$^{+0.23}_{-0.23}$  & 2.94$^{+0.30}_{-0.28}$  & 0.93$^{+0.29}_{-0.26}$ \\
Ca \emissiontype{XIX} He$\beta_{1}$    & 4583.5      & 4583.9$^{+0.4}_{-0.9}$          & 4583.8$^{+0.4}_{-1.0}$ & (fixed)                & (fixed)                   &   & $<$1.5                         & $<$1.4              & (tied)              & (tied)                &   & 0.66$^{+0.16}_{-0.10}$                                     & 0.46$^{+0.13}_{-0.10}$  & 0.49$^{+0.17}_{-0.16}$  & $<$0.15                \\
Ca \emissiontype{XX} Ly$\alpha_{1}$    & 4107.5      & 4107.9$^{+0.3}_{-0.5}$          & 4107.1$^{+0.7}_{-0.4}$ & 4108.4$^{+0.5}_{-0.6}$ & 4113.1$^{+1.8}_{-1.5}$    &   & 2.6$^{+0.4}_{-0.4}$            & 2.9$^{+0.5}_{-0.5}$ & 2.4$^{+0.7}_{-0.6}$ & 3.0$^{+2.1}_{-1.2}$   &   & 2.80$^{+0.18}_{-0.18}$                                     & 1.85$^{+0.16}_{-0.15}$  & 1.81$^{+0.20}_{-0.19}$  & 0.77$^{+0.20}_{-0.19}$ \\
Fe \emissiontype{XXV} w                & 6700.4      & 6700.5$^{+0.1}_{-0.1}$          & 6700.5$^{+0.1}_{-0.1}$ & 6700.5$^{+0.1}_{-0.1}$ & 6701.9$^{+0.2}_{-0.3}$    &   & 4.3$^{+0.1}_{-0.1}$            & 4.5$^{+0.1}_{-0.1}$ & 4.1$^{+0.1}_{-0.1}$ & 4.4$^{+0.2}_{-0.2}$   &   & 34.60$^{+0.41}_{-0.37}$                                    & 22.05$^{+0.32}_{-0.31}$ & 23.03$^{+0.46}_{-0.38}$ & 9.69$^{+0.43}_{-0.46}$ \\
Fe \emissiontype{XXV} z                & 6636.6      & 6636.9$^{+0.1}_{-0.2}$          & 6637.0$^{+0.1}_{-0.2}$ & 6636.9$^{+0.1}_{-0.2}$ & 6637.8$^{+0.4}_{-0.5}$    &   & 3.6$^{+0.1}_{-0.1}$            & 3.8$^{+0.1}_{-0.1}$ & 3.5$^{+0.1}_{-0.2}$ & 3.9$^{+0.5}_{-0.5}$   &   & 13.92$^{+0.28}_{-0.25}$                                    & 9.19$^{+0.22}_{-0.22}$  & 8.89$^{+0.25}_{-0.31}$  & 3.11$^{+0.28}_{-0.27}$ \\
Fe \emissiontype{XXV} He$\beta_{1}$    & 7881.5      & 7881.0$^{+0.2}_{-0.2}$          & 7881.4$^{+0.4}_{-0.3}$ & 7880.8$^{+0.4}_{-0.3}$ & 7882.8$^{+0.5}_{-1.7}$    &   & 4.2$^{+0.2}_{-0.3}$            & 3.6$^{+0.3}_{-0.2}$ & 4.5$^{+0.3}_{-0.3}$ & 4.7$^{+1.1}_{-0.9}$   &   & 4.71$^{+0.15}_{-0.19}$                                     & 2.68$^{+0.15}_{-0.16}$  & 3.42$^{+0.19}_{-0.18}$  & 1.44$^{+0.20}_{-0.20}$ \\
Fe \emissiontype{XXV} He$\beta_{2}$    & 7872.0      & (tied)                          & (tied)                 & (tied)                 & (tied)                    &   & (tied)                         & (tied)              & (tied)              & (tied)                &   & 0.94$^{+0.17}_{-0.10}$                                     & 0.82$^{+0.13}_{-0.12}$  & 0.46$^{+0.13}_{-0.12}$  & $<$0.22                \\
Fe \emissiontype{XXV} He$\gamma_{1}$   & 8295.5      & 8295.3$^{+0.4}_{-0.6}$          & 8295.4$^{+0.7}_{-0.6}$ & 8295.0$^{+0.6}_{-1.1}$ & 8304.6$^{-8304.6}_{-5.3}$ &   & 4.9$^{+0.5}_{-0.5}$            & 4.5$^{+0.7}_{-0.6}$ & 5.4$^{+0.8}_{-0.7}$ & 10.0$^{-10.0}_{-2.0}$ &   & 1.69$^{+0.13}_{-0.12}$                                     & 0.99$^{+0.10}_{-0.10}$  & 1.27$^{+0.14}_{-0.13}$  & 0.44$^{+0.15}_{-0.18}$ \\
Fe \emissiontype{XXV} He$\delta_{1}$   & 8487.4      & 8484.8$^{+1.4}_{-1.2}$          & 8485.7$^{+1.8}_{-1.6}$ & 8483.2$^{+2.1}_{-1.6}$ & 8485.2$^{+1.0}_{-1.3}$    &   & 6.3$^{+1.2}_{-0.9}$            & 6.1$^{+1.6}_{-1.3}$ & 6.6$^{+2.3}_{-1.4}$ & $<$1.9                &   & 0.81$^{+0.12}_{-0.12}$                                     & 0.50$^{+0.10}_{-0.10}$  & 0.57$^{+0.12}_{-0.11}$  & 0.20$^{+0.14}_{-0.06}$ \\
Fe \emissiontype{XXV} He$\epsilon_{1}$ & 8588.5      & 8592.7$^{+1.2}_{-1.5}$          & 8592.7$^{+0.9}_{-2.2}$ & 8594.3$^{+2.9}_{-3.2}$ & 8589.0$^{+3.2}_{-3.6}$    &   & 4.5$^{+1.2}_{-1.0}$            & 3.6$^{+1.5}_{-1.2}$ & 7.1$^{-7.1}_{-2.1}$ & $<$6.4                &   & 0.50$^{+0.10}_{-0.10}$                                     & 0.31$^{+0.08}_{-0.08}$  & 0.38$^{+0.12}_{-0.11}$  & 0.14$^{+0.11}_{-0.09}$ \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$  & 6973.1      & 6973.6$^{+0.1}_{-0.5}$          & 6973.3$^{+0.4}_{-0.4}$ & 6973.6$^{+0.2}_{-0.5}$ & 6973.9$^{+1.1}_{-1.7}$    &   & 4.2$^{+0.2}_{-0.2}$            & 4.6$^{+0.3}_{-0.3}$ & 3.8$^{+0.2}_{-0.4}$ & 6.2$^{+1.2}_{-0.9}$   &   & 3.55$^{+0.16}_{-0.16}$                                     & 2.15$^{+0.14}_{-0.13}$  & 2.59$^{+0.18}_{-0.16}$  & 1.35$^{+0.22}_{-0.21}$ \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$  & 6951.9      & 6952.9$^{+0.2}_{-0.6}$          & 6952.9$^{+0.4}_{-0.9}$ & 6952.7$^{+0.4}_{-0.5}$ & 6953.1$^{+1.4}_{-1.9}$    &   & (tied)                         & (tied)              & (tied)              & (tied)                &   & 2.14$^{+0.14}_{-0.13}$                                     & 1.29$^{+0.12}_{-0.11}$  & 1.56$^{+0.14}_{-0.14}$  & 0.99$^{+0.20}_{-0.18}$ \\
Fe \emissiontype{XXVI} Ly$\beta_{1}$   & 8252.6      & 8255.2$^{+1.0}_{-1.3}$          & 8254.5$^{+1.7}_{-1.7}$ & 8256.0$^{+0.3}_{-1.9}$ & 8250.5$^{+1.6}_{-3.6}$    &   & $<$3.3                         & 2.4$^{+2.4}_{-1.1}$ & $<$2.2              & $<$5.2                &   & 0.28$^{+0.06}_{-0.06}$                                     & 0.18$^{+0.05}_{-0.05}$  & 0.17$^{+0.07}_{-0.04}$  & 0.17$^{+0.08}_{-0.07}$ \\
Fe \emissiontype{XXVII} w              & 7805.6      & 7806.8$^{+0.6}_{-0.9}$          & 7806.7$^{+1.2}_{-0.6}$ & 7805.6$^{+1.7}_{-1.3}$ & 7803.7$^{+2.5}_{-4.0}$    &   & 6.1$^{+0.8}_{-0.9}$            & 5.7$^{+1.0}_{-0.9}$ & 6.9$^{+1.7}_{-1.4}$ & 6.7$^{-6.7}_{-2.3}$   &   & 1.55$^{+0.13}_{-0.14}$                                     & 1.06$^{+0.12}_{-0.11}$  & 0.89$^{+0.14}_{-0.13}$  & 0.45$^{+0.16}_{-0.15}$ \\
\hline
\end{tabular}
}\label{tab:linedata}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip%
The Ly$\alpha_2$ lines of Si, S, Ar, and Ca are not shown because all the paramters of them are tied to Ly$\alpha_1$ (see \Tab{tab:linelist} for details).\end{tabnote}\end{table}
\end{landscape}

==> tables/linefluxnew.tex.20170804 <==

\begin{table}[]
\tbl{Observed line fluxes derived from the Gaussian fits.\footnotemark[$*$]}{%
\centering
\scriptsize
\begin{tabular}{lrrrr}
\hline
\multicolumn{1}{c}{Line name}          & \multicolumn{4}{c}{Flux (10$^{-5}$~ph~cm$^ {-2}$~s$^ {-1}$)} \\
\cline{2-5}                            & \multicolumn{1}{c}{Entire Core}                              & \multicolumn{1}{c}{Nebula} & \multicolumn{1}{c}{Rim}     & \multicolumn{1}{c}{Outer}   \\
\hline
Si \emissiontype{XIII} w               & 7.19$^{+3.77}_{-3.42}$                                       & 5.83$^{+3.63}_{-2.51}$     & \multicolumn{1}{c}{$<$5.44} & \multicolumn{1}{c}{$<$4.58} \\
Si \emissiontype{XIV} Ly$\alpha_{1}$   & 31.90$^{+2.28}_{-2.21}$                                      & 20.10$^{+1.92}_{-1.82}$    & 21.82$^{+2.64}_{-2.52}$     & 4.04$^{+2.09}_{-1.67}$      \\
Si \emissiontype{XIV} Ly$\beta_{1}$    & 6.89$^{+0.89}_{-0.86}$                                       & 5.03$^{+0.74}_{-0.70}$     & 3.93$^{+1.04}_{-0.98}$      & 1.23$^{+0.80}_{-0.60}$      \\
S \emissiontype{XV} w                  & 9.21$^{+1.10}_{-1.11}$                                       & 7.26$^{+0.98}_{-0.99}$     & 3.91$^{+1.03}_{-0.94}$      & \multicolumn{1}{c}{$<$1.08} \\
S \emissiontype{XVI} Ly$\alpha_{1}$    & 22.32$^{+0.73}_{-0.72}$                                      & 15.81$^{+0.64}_{-0.63}$    & 12.46$^{+0.77}_{-0.76}$     & 2.70$^{+0.68}_{-0.61}$      \\
S \emissiontype{XVI} Ly$\beta_{1}$     & 3.83$^{+0.29}_{-0.29}$                                       & 2.55$^{+0.25}_{-0.24}$     & 2.49$^{+0.34}_{-0.33}$      & 0.63$^{+0.26}_{-0.23}$      \\
S \emissiontype{XVI} Ly$\gamma_{1}$    & 1.20$^{+0.20}_{-0.19}$                                       & 0.79$^{+0.09}_{-0.25}$     & 0.92$^{+0.25}_{-0.24}$      & 0.32$^{+0.22}_{-0.17}$      \\
Ar \emissiontype{XVII} w               & 3.72$^{+0.37}_{-0.36}$                                       & 2.82$^{+0.31}_{-0.30}$     & 1.88$^{+0.51}_{-0.47}$      & 1.20$^{+0.42}_{-0.34}$      \\
Ar \emissiontype{XVIII} Ly$\alpha_{1}$ & 5.47$^{+0.29}_{-0.29}$                                       & 3.85$^{+0.25}_{-0.25}$     & 3.16$^{+0.32}_{-0.30}$      & 0.95$^{+0.32}_{-0.30}$      \\
Ar \emissiontype{XVIII} Ly$\beta_{1}$  & 0.77$^{+0.15}_{-0.15}$                                       & 0.51$^{+0.12}_{-0.12}$     & 0.63$^{+0.20}_{-0.18}$      & 0.26$^{+0.15}_{-0.11}$      \\
Ca \emissiontype{XIX} w                & 5.20$^{+0.27}_{-0.27}$                                       & 3.66$^{+0.23}_{-0.23}$     & 2.94$^{+0.30}_{-0.28}$      & 0.93$^{+0.29}_{-0.26}$      \\
Ca \emissiontype{XIX} He$\beta_{1}$    & 0.66$^{+0.16}_{-0.10}$                                       & 0.46$^{+0.13}_{-0.10}$     & 0.49$^{+0.17}_{-0.16}$      & \multicolumn{1}{c}{$<$0.15} \\
Ca \emissiontype{XX} Ly$\alpha_{1}$    & 2.80$^{+0.18}_{-0.18}$                                       & 1.85$^{+0.16}_{-0.15}$     & 1.81$^{+0.20}_{-0.19}$      & 0.77$^{+0.20}_{-0.19}$      \\
Fe \emissiontype{XXV} w                & 34.60$^{+0.41}_{-0.37}$                                      & 22.05$^{+0.32}_{-0.31}$    & 23.03$^{+0.46}_{-0.38}$     & 9.68$^{+0.44}_{-0.45}$      \\
Fe \emissiontype{XXV} z                & 13.92$^{+0.28}_{-0.25}$                                      & 9.19$^{+0.22}_{-0.22}$     & 8.89$^{+0.25}_{-0.31}$      & 3.11$^{+0.28}_{-0.27}$      \\
Fe \emissiontype{XXV} He$\beta_{1}$    & 4.71$^{+0.15}_{-0.19}$                                       & 2.68$^{+0.15}_{-0.16}$     & 3.42$^{+0.19}_{-0.18}$      & 1.52$^{+0.20}_{-0.23}$      \\
Fe \emissiontype{XXV} He$\beta_{2}$    & 0.94$^{+0.17}_{-0.10}$                                       & 0.82$^{+0.13}_{-0.12}$     & 0.46$^{+0.13}_{-0.12}$      & \multicolumn{1}{c}{$<$0.14} \\
Fe \emissiontype{XXV} He$\gamma_{1}$   & 1.69$^{+0.13}_{-0.12}$                                       & 0.99$^{+0.10}_{-0.10}$     & 1.27$^{+0.14}_{-0.13}$      & 0.24$^{+0.14}_{-0.12}$      \\
Fe \emissiontype{XXV} He$\delta_{1}$   & 0.81$^{+0.12}_{-0.12}$                                       & 0.50$^{+0.10}_{-0.10}$     & 0.57$^{+0.12}_{-0.11}$      & 0.27$^{+0.13}_{-0.11}$      \\
Fe \emissiontype{XXV} He$\epsilon_{1}$ & 0.50$^{+0.10}_{-0.10}$                                       & 0.31$^{+0.08}_{-0.08}$     & 0.38$^{+0.12}_{-0.11}$      & 0.14$^{+0.12}_{-0.10}$      \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$  & 3.55$^{+0.16}_{-0.16}$                                       & 2.15$^{+0.14}_{-0.13}$     & 2.59$^{+0.18}_{-0.16}$      & 1.34$^{+0.23}_{-0.21}$      \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$  & 2.14$^{+0.14}_{-0.13}$                                       & 1.29$^{+0.12}_{-0.11}$     & 1.56$^{+0.14}_{-0.14}$      & 0.99$^{+0.20}_{-0.19}$      \\
Fe \emissiontype{XXVI} Ly$\beta_{1}$   & 0.28$^{+0.06}_{-0.06}$                                       & 0.18$^{+0.05}_{-0.05}$     & 0.17$^{+0.07}_{-0.04}$      & 0.17$^{+0.08}_{-0.07}$      \\
Ni \emissiontype{XXVII} w              & 1.55$^{+0.13}_{-0.14}$                                       & 1.06$^{+0.12}_{-0.11}$     & 0.89$^{+0.14}_{-0.13}$      & 0.44$^{+0.17}_{-0.15}$      \\
\hline
\end{tabular}
}\label{tab:linedata}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip%
The Ly$\alpha_2$ lines of Si, S, Ar, and Ca are not shown because all the paramters of them are tied to Ly$\alpha_1$ (see \Tab{tab:linelist} for details).
\end{tabnote}\end{table}


==> tables/linefluxnew2.tex.20170804 <==

\begin{table*}[]
\tbl{Observed line centers and widths derived from the Gaussian fits..\footnotemark[$*$]}{%
\centering
\scriptsize
\begin{tabular}{lcrrrrcrrrr}
\hline
\multicolumn{1}{c}{Line name}          & \multicolumn{1}{c}{$E_0$~(eV)\footnotemark[$\dagger$]} & \multicolumn{4}{c}{Center (eV)} && \multicolumn{4}{c}{Width (eV)}  \\
\cline{3-6}\cline{8-11}                &                                                        & \multicolumn{1}{c}{Entire Core} & \multicolumn{1}{c}{Nebula} & \multicolumn{1}{c}{Rim}     & \multicolumn{1}{c}{Outer}   & ~ & \multicolumn{1}{c}{Entire Core} & \multicolumn{1}{c}{Nebula} & \multicolumn{1}{c}{Rim}    & \multicolumn{1}{c}{Outer}  \\
\hline
Si \emissiontype{XIII} w               & 1865.0                                                 & 1864.6$^{+1.0}_{-1.1}$          & 1864.2$^{+1.5}_{-1.0}$     & \multicolumn{1}{c}{(fixed)} & \multicolumn{1}{c}{(fixed)} &   & \multicolumn{1}{c}{$<$1.7}      & \multicolumn{1}{c}{$<$1.7} & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} \\
Si \emissiontype{XIV} Ly$\alpha_{1}$   & 2006.1                                                 & 2006.4$^{+0.3}_{-0.2}$          & 2006.5$^{+0.3}_{-0.2}$     & 2006.4$^{+0.4}_{-0.3}$      & 2006.4$^{+1.4}_{-1.4}$      &   & 1.3$^{+0.3}_{-0.3}$             & \multicolumn{1}{c}{$<$1.5} & 1.7$^{+0.5}_{-0.5}$        & \multicolumn{1}{c}{$<$2.8} \\
Si \emissiontype{XIV} Ly$\beta_{1}$    & 2376.6                                                 & 2376.5$^{+0.5}_{-0.5}$          & 2376.2$^{+0.5}_{-0.5}$     & 2377.8$^{+1.3}_{-1.4}$      & 2378.5$^{+1.0}_{-1.4}$      &   & 2.4$^{+0.5}_{-0.5}$             & 2.2$^{+0.5}_{-0.5}$        & 3.8$^{+1.3}_{-1.2}$        & \multicolumn{1}{c}{$<$2.0} \\
S \emissiontype{XV} w                  & 2460.6                                                 & 2460.7$^{+0.5}_{-0.3}$          & 2460.6$^{+0.6}_{-0.4}$     & 2460.7$^{+0.8}_{-0.6}$      & \multicolumn{1}{c}{(fixed)} &   & 2.1$^{+0.6}_{-0.6}$             & 2.6$^{+0.8}_{-0.7}$        & \multicolumn{1}{c}{$<$2.2} & \multicolumn{1}{c}{(tied)} \\
S \emissiontype{XVI} Ly$\alpha_{1}$    & 2622.7                                                 & 2622.6$^{+0.1}_{-0.1}$          & 2622.7$^{+0.1}_{-0.2}$     & 2622.6$^{+0.2}_{-0.2}$      & 2621.6$^{+0.9}_{-0.9}$      &   & 1.8$^{+0.2}_{-0.2}$             & 1.9$^{+0.2}_{-0.2}$        & 1.7$^{+0.3}_{-0.3}$        & 2.0$^{+1.0}_{-1.1}$        \\
S \emissiontype{XVI} Ly$\beta_{1}$     & 3106.7                                                 & 3106.4$^{+0.3}_{-0.3}$          & 3106.0$^{+0.4}_{-0.4}$     & 3107.0$^{+0.3}_{-0.5}$      & 3116.1$^{+0.7}_{-1.3}$      &   & 2.1$^{+0.4}_{-0.3}$             & 2.4$^{+0.5}_{-0.4}$        & 1.8$^{+0.5}_{-0.7}$        & \multicolumn{1}{c}{$<$1.8} \\
S \emissiontype{XVI} Ly$\gamma_{1}$    & 3276.3                                                 & 3276.8$^{+0.3}_{-0.8}$          & 3276.8$^{+0.4}_{-0.9}$     & 3276.3$^{+1.0}_{-0.8}$      & 3275.7$^{+1.4}_{-1.5}$      &   & \multicolumn{1}{c}{$<$2.0}      & \multicolumn{1}{c}{$<$2.4} & 1.8$^{+1.2}_{-1.4}$        & \multicolumn{1}{c}{$<$2.4} \\
Ar \emissiontype{XVII} w               & 3139.6                                                 & 3139.5$^{+0.3}_{-0.3}$          & 3139.5$^{+0.3}_{-0.4}$     & 3139.3$^{+1.2}_{-1.1}$      & 3142.4$^{+0.7}_{-0.9}$      &   & 1.5$^{+0.4}_{-0.4}$             & 1.1$^{+0.5}_{-0.6}$        & 3.0$^{+1.4}_{-1.1}$        & \multicolumn{1}{c}{$<$1.9} \\
Ar \emissiontype{XVIII} Ly$\alpha_{1}$ & 3323.0                                                 & 3322.9$^{+0.2}_{-0.3}$          & 3323.1$^{+0.3}_{-0.4}$     & 3322.5$^{+0.5}_{-0.4}$      & 3326.6$^{+2.2}_{-2.2}$      &   & 2.7$^{+0.4}_{-0.4}$             & 3.0$^{+0.4}_{-0.4}$        & 2.2$^{+0.6}_{-0.6}$        & 4.2$^{+2.3}_{-1.6}$        \\
Ar \emissiontype{XVIII} Ly$\beta_{1}$  & 3935.7                                                 & 3935.0$^{+0.9}_{-1.0}$          & 3936.2$^{+0.7}_{-1.3}$     & 3931.4$^{+1.5}_{-1.7}$      & 3946.6$^{+0.7}_{-1.2}$      &   & 2.8$^{+1.0}_{-0.8}$             & 2.3$^{+1.0}_{-0.9}$        & 3.7$^{+1.7}_{-1.6}$        & \multicolumn{1}{c}{$<$1.2} \\
Ca \emissiontype{XIX} w                & 3902.4                                                 & 3902.4$^{+0.2}_{-0.2}$          & 3902.5$^{+0.2}_{-0.3}$     & 3902.1$^{+0.3}_{-0.4}$      & 3902.4$^{+1.5}_{-1.1}$      &   & 2.3$^{+0.2}_{-0.2}$             & 2.4$^{+0.3}_{-0.3}$        & 2.2$^{+0.4}_{-0.4}$        & 2.7$^{+1.5}_{-1.2}$        \\
Ca \emissiontype{XIX} He$\beta_{1}$    & 4583.5                                                 & 4583.9$^{+0.4}_{-0.9}$          & 4583.8$^{+0.4}_{-1.0}$     & \multicolumn{1}{c}{(fixed)} & \multicolumn{1}{c}{(fixed)} &   & \multicolumn{1}{c}{$<$1.5}      & \multicolumn{1}{c}{$<$1.4} & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} \\
Ca \emissiontype{XX} Ly$\alpha_{1}$    & 4107.5                                                 & 4107.9$^{+0.3}_{-0.5}$          & 4107.1$^{+0.7}_{-0.4}$     & 4108.4$^{+0.5}_{-0.6}$      & 4113.1$^{+1.8}_{-1.5}$      &   & 2.6$^{+0.4}_{-0.4}$             & 2.9$^{+0.5}_{-0.5}$        & 2.4$^{+0.7}_{-0.6}$        & 3.0$^{+2.1}_{-1.2}$        \\
Fe \emissiontype{XXV} w                & 6700.4                                                 & 6700.5$^{+0.1}_{-0.1}$          & 6700.5$^{+0.1}_{-0.1}$     & 6700.5$^{+0.1}_{-0.1}$      & 6701.9$^{+0.2}_{-0.3}$      &   & 4.3$^{+0.1}_{-0.1}$             & 4.5$^{+0.1}_{-0.1}$        & 4.1$^{+0.1}_{-0.1}$        & 4.4$^{+0.2}_{-0.2}$        \\
Fe \emissiontype{XXV} z                & 6636.6                                                 & 6636.9$^{+0.1}_{-0.2}$          & 6637.0$^{+0.1}_{-0.2}$     & 6636.9$^{+0.1}_{-0.2}$      & 6637.8$^{+0.4}_{-0.5}$      &   & 3.6$^{+0.1}_{-0.1}$             & 3.8$^{+0.1}_{-0.1}$        & 3.5$^{+0.1}_{-0.2}$        & 3.9$^{+0.5}_{-0.5}$        \\
Fe \emissiontype{XXV} He$\beta_{1}$    & 7881.5                                                 & 7881.0$^{+0.2}_{-0.2}$          & 7881.4$^{+0.4}_{-0.3}$     & 7880.8$^{+0.4}_{-0.3}$      & 7882.2$^{+0.7}_{-1.2}$      &   & 4.2$^{+0.2}_{-0.3}$             & 3.6$^{+0.3}_{-0.2}$        & 4.5$^{+0.3}_{-0.3}$        & 5.0$^{+0.9}_{-0.8}$        \\
Fe \emissiontype{XXV} He$\beta_{2}$    & 7872.0                                                 & \multicolumn{1}{c}{(tied)}      & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)}  & \multicolumn{1}{c}{(tied)}  &   & \multicolumn{1}{c}{(tied)}      & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} \\
Fe \emissiontype{XXV} He$\gamma_{1}$   & 8295.5                                                 & 8295.3$^{+0.4}_{-0.6}$          & 8295.4$^{+0.7}_{-0.6}$     & 8295.0$^{+0.6}_{-1.1}$      & \multicolumn{1}{c}{(fixed)} &   & 4.9$^{+0.5}_{-0.5}$             & 4.5$^{+0.7}_{-0.6}$        & 5.4$^{+0.8}_{-0.7}$        & \multicolumn{1}{c}{$<$0.0} \\
Fe \emissiontype{XXV} He$\delta_{1}$   & 8487.4                                                 & 8484.8$^{+1.4}_{-1.2}$          & 8485.7$^{+1.8}_{-1.6}$     & 8483.2$^{+2.1}_{-1.6}$      & \multicolumn{1}{c}{(fixed)} &   & 6.3$^{+1.2}_{-0.9}$             & 6.1$^{+1.6}_{-1.3}$        & 6.6$^{+2.3}_{-1.4}$        & \multicolumn{1}{c}{$<$0.0} \\
Fe \emissiontype{XXV} He$\epsilon_{1}$ & 8588.5                                                 & 8592.7$^{+1.2}_{-1.5}$          & 8592.7$^{+0.9}_{-2.2}$     & 8594.3$^{+2.9}_{-3.2}$      & \multicolumn{1}{c}{(fixed)} &   & 4.5$^{+1.2}_{-1.0}$             & 3.6$^{+1.5}_{-1.2}$        & 7.1$^{-7.1}_{-2.1}$        & \multicolumn{1}{c}{$<$0.0} \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$  & 6973.1                                                 & 6973.6$^{+0.1}_{-0.5}$          & 6973.3$^{+0.4}_{-0.4}$     & 6973.6$^{+0.2}_{-0.5}$      & 6973.9$^{+1.1}_{-1.7}$      &   & 4.2$^{+0.2}_{-0.2}$             & 4.6$^{+0.3}_{-0.3}$        & 3.8$^{+0.2}_{-0.4}$        & 6.1$^{+1.2}_{-0.9}$        \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$  & 6951.9                                                 & 6952.9$^{+0.2}_{-0.6}$          & 6952.9$^{+0.4}_{-0.9}$     & 6952.7$^{+0.4}_{-0.5}$      & 6953.1$^{+1.4}_{-2.0}$      &   & \multicolumn{1}{c}{(tied)}      & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} & \multicolumn{1}{c}{(tied)} \\
Fe \emissiontype{XXVI} Ly$\beta_{1}$   & 8252.6                                                 & 8255.2$^{+1.0}_{-1.3}$          & 8254.5$^{+1.7}_{-1.7}$     & 8256.0$^{+0.3}_{-1.9}$      & 8250.7$^{+1.6}_{-4.0}$      &   & \multicolumn{1}{c}{$<$3.3}      & 2.4$^{+2.4}_{-1.1}$        & \multicolumn{1}{c}{$<$2.2} & \multicolumn{1}{c}{$<$5.4} \\
Ni \emissiontype{XXVII} w              & 7805.6                                                 & 7806.8$^{+0.6}_{-0.9}$          & 7806.7$^{+1.2}_{-0.6}$     & 7805.6$^{+1.7}_{-1.3}$      & 7803.7$^{+2.8}_{-4.0}$      &   & 6.1$^{+0.8}_{-0.9}$             & 5.7$^{+1.0}_{-0.9}$        & 6.9$^{+1.7}_{-1.4}$        & 6.6$^{+3.8}_{-2.4}$        \\
\hline
\end{tabular}
}\label{tab:linedata2}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip%
The Ly$\alpha_2$ lines of Si, S, Ar, and Ca are not shown because all the paramters of them are tied to Ly$\alpha_1$ (see \Tab{tab:linelist} for details).
\par
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$\dagger$]\hss}\unskip%
Fiducial energies of the lines at the rest frame. 
\end{tabnote}\end{table*}


==> tables/linelist.tex.20170720 <==
\begin{table}[]
\tbl{List of considered lines for the Gaussian fit.\footnotemark[$*$]}{%
\centering
\scriptsize
\begin{tabular}{llccc}
\hline
\multicolumn{1}{c}{Line name}                            &  \multicolumn{4}{c}{Constraints}                                                \\
\cline{2-5}
                            & \multicolumn{1}{c}{Tied to}                            & \multicolumn{1}{c}{Center}                                             & \multicolumn{1}{c}{Width}                                  & \multicolumn{1}{c}{Flux}                                                \\
\hline
Si \emissiontype{XIII} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\alpha_{2}$ &   Si \emissiontype{XIV} Ly$\alpha_{1}$ &$- 1.8$ eV & $\times 1.0$  & $\times 0.5$ \\
Si \emissiontype{XIV} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Si \emissiontype{XIV} Ly$\beta_{2}$ &   Si \emissiontype{XIV} Ly$\beta_{1}$ &$- 0.5$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XV} w &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\alpha_{2}$ &   S \emissiontype{XVI} Ly$\alpha_{1}$ &$- 3.0$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XVI} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\beta_{2}$ &   S \emissiontype{XVI} Ly$\beta_{1}$ &$- 0.9$ eV & $\times 1.0$  & $\times 0.5$ \\
S \emissiontype{XVI} Ly$\gamma_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
S \emissiontype{XVI} Ly$\gamma_{2}$ &   S \emissiontype{XVI} Ly$\gamma_{1}$ &$- 0.4$ eV & $\times 1.0$  & $\times 0.5$ \\
Ar \emissiontype{XVII} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\alpha_{2}$ &   Ar \emissiontype{XVIII} Ly$\alpha_{1}$ & $- 4.8$ eV & $\times 1.0$  & $\times 0.5$ \\
Ar \emissiontype{XVIII} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ar \emissiontype{XVIII} Ly$\beta_{2}$ &   Ar \emissiontype{XVIII} Ly$\beta_{1}$&$- 1.4$ eV &  $\times 1.0$ & $\times 0.5$ \\
Ca \emissiontype{XIX} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XIX} He$\beta_{1}$\footnotemark[$\dagger$] &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XX} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Ca \emissiontype{XX} Ly$\alpha_{2}$ &   Ca \emissiontype{XX} Ly$\alpha_{1}$&$- 7.4$ eV & $\times 1.0$  & $\times 0.5$ \\
Fe \emissiontype{XXV} z &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} w &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\beta_{2}$ &   Fe \emissiontype{XXV} He$\beta_{1}$&$- 9.5$ eV & $\times 1.0$  & - \\
Fe \emissiontype{XXV} He$\gamma_{1}$\footnotemark[$\dagger$] &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\delta_{1}$\footnotemark[$\dagger$] &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXV} He$\epsilon_{1}$\footnotemark[$\dagger$] &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXVI} Ly$\alpha_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXVI} Ly$\alpha_{2}$ & Fe \emissiontype{XXVI} Ly$\alpha_{1}$&  - & $\times 1.0$  & - \\
Fe \emissiontype{XXVI} Ly$\beta_{1}$ &   \multicolumn{1}{c}{-} & - & -  & - \\
Fe \emissiontype{XXVI} Ly$\beta_{2}$ & Fe \emissiontype{XXVI} Ly$\beta_{1}$& $- 6.2$ eV & $\times 1.0$  & - \\
Ni \emissiontype{XXVII} w &   \multicolumn{1}{c}{-} & - & -  & - \\
\hline
\multicolumn{5}{c}{Constraints only on the Rim region} \\
Si \emissiontype{XIII} w &   Si \emissiontype{XIV} Ly$\alpha_{1}$ & fixed at 1865.0 eV & $\times 1.0$  & - \\
Ca \emissiontype{XIX} He$\beta_{1}$ &  Ca \emissiontype{XX} Ly$\alpha_{1}$& fixed at 4583.5 eV &  $\times 1.0$ & - \\
\hline
\multicolumn{5}{c}{Constraints only on the Outer region} \\
Si \emissiontype{XIII} w &   Si \emissiontype{XIV} Ly$\alpha_{1}$& fixed at 1865.0 eV & $\times 1.0$  & - \\
S \emissiontype{XV} w &   S \emissiontype{XVI} Ly$\alpha_{1}$&fixed at 2460.6 eV&  $\times 1.0$ & - \\
Ca \emissiontype{XIX} He$\beta_{1}$ & Ca \emissiontype{XX} Ly$\alpha_{1}$& fixed at  4583.5 eV & $\times 1.0$  & - \\
Fe \emissiontype{XXV} He$\gamma_{1}$ & Fe \emissiontype{XXV} He$\beta_{1}$ & fixed at  8295.5 eV & $\times 1.0$  & - \\
Fe \emissiontype{XXV} He$\delta_{1}$ & Fe \emissiontype{XXV} He$\beta_{1}$ & fixed at  8487.4 eV & $\times 1.0$  & - \\
Fe \emissiontype{XXV} He$\epsilon_{1}$ & Fe \emissiontype{XXV} He$\beta_{1}$ & fixed at  8588.5 eV & $\times 1.0$  & - \\
\hline
\end{tabular}
}\label{tab:linelist}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip% 
Free parameters are denoted by the hyphen (-).
\par\noindent
\hbox to6pt{\footnotemark[$\dagger$]\hss}\unskip% 
Ca \emissiontype{XIX} He$\beta_{2}$, Fe \emissiontype{XXV} He$\gamma_{2}$, Fe \emissiontype{XXV} He$\delta_{2}$, and Fe \emissiontype{XXV} He$\epsilon_{2}$ were omitted because their fluxes are too small to constrain from the SXS spetra.
\end{tabnote}
\end{table}


==> tables/observations.tex.20170724 <==
\begin{table*}
  \tbl{Observation logs.}{%
  \begin{tabular}{clcccc}
      \hline
      Name & \multicolumn{1}{c}{Observation ID} & $\alpha_{2000.0}$ & $\delta_{2000.0}$  & Observation Date & Effective Exposure \\ 
      &  & (deg) & (deg) &  & (ks) \\ 
      \hline
      obs1 & 100040010 & 49.878 & 41.484 & 2016-02-24 -- 2016-02-25 & 48.7 \\
      obs2 & 100040020 & 49.935 & 41.519 & 2016-02-25 -- 2016-02-27 & 97.4 \\
      obs3 & 100040030, 100040040, 100040050& 49.936 & 41.520 & 2016-03-04 -- 2016-03-06 & 146.1 \\
      obs4 & 100040060 & 49.955 & 41.512 & 2016-03-06 -- 2016-03-07 & 45.8 \\
      \hline
    \end{tabular}}\label{tab:obslog}
\end{table*}


==> tables/powerlaw.tex <==
\begin{table}[]
\tbl{Surface brightness of the power-law component.\footnotemark[$*$]}{%
\centering
\begin{tabular}{@{\extracolsep{4pt}}lcccccc}
\hline
Instrument             & \multicolumn{2}{c}{AtomDB 3.0.9} & \multicolumn{2}{c}{SPEXACT 3.03.00} \\
\cline{2-3}\cline{4-5} & Nebula                              & Rim                       & Nebula                               & Rim      \\
\hline
Hitomi/SXS             & $<$2.2                              & $<$1.2                    & $<$2.7                             & $<$0.7 \\
Chandra/ACIS         & $6.3_{-0.5}^{+0.5}$                 & $2.0_{-0.3}^{+0.3}$       & $6.6_{-0.5}^{+0.5}$                & $1.9_{-0.3}^{+0.3}$ \\
\hline
\end{tabular}
}\label{tab:powerlaw}
\begin{tabnote}
\hangindent6pt\noindent
\hbox to6pt{\footnotemark[$*$]\hss}\unskip%
In the unit of 10$^{-16}~$~erg~cm$^{-2}$~s$^{-1}$~arcsec$^{-2}$ (2--10~keV band)
\end{tabnote}\end{table}


==> tables/systematic.tex <==

\begin{table}[]
\centering
\scriptsize
\caption{Systematic uncertainties due to different effective areas}
\label{tab:systematic}
\begin{tabular}{lccccc}
\hline
\multicolumn{1}{c}{Regin/Correction} & $kT_{1}$ & Norm$_{1}$ & $kT_{2}$ & Norm$_{2}$ & $kT_{\rm cont}$ \\ \hline
Center                               &          &            &          &            &                 \\
~~Ground cal.                        & 0.9\% & -4.7\% & -4.5\% & 18.7\% & -2.0\% \\
~~Crab ratio                         & 0.3\% & 1.9\% & -2.5\% & -3.0\% & 10.9\% \\ \hline
N                                    &          &            &          &            &                 \\
~~Ground cal.                        & 0.7\% & -4.7\% & -0.3\% & 26.9\% & -0.1\% \\
~~Crab ratio                         & 0.4\% & 1.7\% & -0.4\% & -1.5\% & 6.3\% \\ \hline
NW                                   &          &            &          &            &                 \\
~~Ground cal.                        & -0.0\% & -2.8\% & -17.4\% & -3.8\% & -0.1\% \\
~~Crab ratio                         & -0.3\% & 3.2\% & -14.7\% & -15.6\% & 7.3\% \\ \hline
W                                    &          &            &          &            &                 \\
~~Ground cal.                        & 1.4\% & -5.8\% & (fixed) & -5.4\% & -0.1\%  \\
~~Crab ratio                         & 0.5\% & 1.5\% & (fixed) & 7.2\% & 6.2\% \\ \hline
SE                                   &          &            &          &            &                 \\
~~Ground cal.                        & 0.3\% & -4.3\% & (fixed) & 4.1\% & -0.2\% \\
~~Crab ratio                         & 0.5\% & 1.6\% & (fixed) & 0.2\% & 6.2\% \\ \hline
Far W                                &          &            &          &            &                 \\
~~Ground cal.                        & 0.5\% & -4.1\% & (fixed) & 35.0\% & 0.6\% \\
~~Crab ratio                         & 0.4\% & 1.8\% & (fixed) & 6.5\% & 7.1\% \\ \hline
\end{tabular}
\end{table}


